InclusiViz: Visual Analytics of Human Mobility Data for Understanding and Mitigating Urban Segregation

Urban segregation refers to the physical and social division of people, often driving inequalities within cities and exacerbating socioeconomic and racial tensions. While most studies focus on residential spaces, they often neglect segregation across "activity spaces" where people work, socialize, and engage in leisure. Human mobility data offers new opportunities to analyze broader segregation patterns, encompassing both residential and activity spaces, but challenges existing methods in capturing the complexity and local nuances of urban segregation. This work introduces InclusiViz, a novel visual analytics system for multi-level analysis of urban segregation, facilitating the development of targeted, data-driven interventions. Specifically, we developed a deep learning model to predict mobility patterns across social groups using environmental features, augmented with explainable AI to reveal how these features influence segregation. The system integrates innovative visualizations that allow users to explore segregation patterns from broad overviews to fine-grained detail and evaluate urban planning interventions with real-time feedback. We conducted a quantitative evaluation to validate the model's accuracy and efficiency. Two case studies and expert interviews with social scientists and urban analysts demonstrated the system's effectiveness, highlighting its potential to guide urban planning toward more inclusive cities.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> archive/sections_for_pvis25_first_sub/00_abstract.tex <==
% dyu
\abstract{
\dyu{Urban segregation refers to the physical and social division of people, often leading to inequalities within cities and even exacerbating socioeconomic and racial tensions. Most segregation studies focus on residential spaces, overlooking segregation dynamics across ``activity spaces'' where people engage in work, leisure, and social interactions. GPS-based human mobility data provides new insights into broader segregation patterns by involving both residential and activity spaces but poses new challenges to existing statistical methods in capturing urban segregation's complexity and local nuances.}
% Urban segregation is an increasingly critical social problem, creating invisible barriers that exacerbate social inequalities within cities. 
% Existing segregation studies, which predominantly focus on residential areas, fail to fully capture the complex dynamics of segregation across various ``activity spaces'' such as work, leisure, and social interactions.
% The proliferation of GPS-based human mobility data offers a fresh perspective for a detailed analysis of segregation within a broader area, but it also introduces challenges to existing statistical approaches in understanding the complex dynamics and local nuances of urban segregation. 
This work introduces \systemname, a novel visual analytics system that enables comprehensive and multi-level analyses of urban segregation and \dyu{facilitates} the development of targeted, data-driven interventions and policy-making. 
Specifically, we developed a deep learning model to predict mobility patterns across different social groups using environmental features, enhanced with explainable AI to uncover how these features influence the degree of segregation. % segregation levels. 
% reveal the impacts of these features on segregation levels. 
The system integrates a set of innovative visualizations that empower users to explore segregation patterns from broad overviews to fine-grained detail and further develop and evaluate urban planning interventions with real-time feedback. 
We conduct a quantitative evaluation to demonstrate the accuracy and time complexity of our \yy{model}. 
Two case studies and expert interviews with social scientists and urban analysts demonstrated the effectiveness and usefulness of our system, 
% are further conducted to validate our system's efficacy, 
confirming its potential to significantly inform and guide urban planning efforts toward creating more inclusive and equitable urban environments.
}

% V2.0
% \abstract{
% Segregation is a critical social problem, isolating a city into filter bubbles that limit opportunities and hinder social equality. 
% While traditional approaches analyze residential segregation, the emergence of large-scale human mobility data allows more fine-grained segregation study within ``activity spaces'' (\eg, work, leisure, and social areas).
% However, existing social science methods fall short in this data with a focus on global statistics, lacking detailed insights for holistic understanding and simulation for informed policy-making.
% This work introduces \systemname, an interactive visual analytics system that empowers social scientists and policymakers to conduct multi-level segregation analyses and develop data-driven interventions to mitigate segregation. 
% \systemname leverages a deep learning model to predict mobility patterns across social groups based on environmental features, while explainable AI techniques reveal feature impacts on segregation levels.
% In addition, a suite of coordinated visualization views is proposed to aid exploration. 
% Experts can explore how environmental features shape local spatial interactions and dynamically adjust features to receive real-time feedback on the interface, facilitating an iterative process to refine data-driven interventions.
% We conduct a quantitative evaluation to show the accuracy of our algorithm.
% Two case studies and expert interviews with social scientists and urban analysts are further conducted to validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive environments.
% }

% V1.0
% \abstract{
% Segregation is a critical social problem, isolating a city into different filter bubbles that hamper community integration and limit opportunities for underprivileged groups. 
% This makes understanding and mitigating segregation a vital goal for social scientists and policymakers to foster social equality.
% Recently, the emergence of large-scale human mobility data has provided new opportunities to study fine-grained segregation within ``activity spaces'' — areas where people work, socialize, and leisure beyond traditional residential locations.
% However, despite this data availability, existing approaches remain limited by their focus on global statistics, lacking detailed insights for holistic understanding and effective simulation for feedback-driven policy-making.
% Hence, in this study, we address this gap by introducing \systemname, an interactive visual analytics system that empowers social scientists and policymakers to conduct nuanced analyses of urban segregation and to develop effective interventions through simulation-driven insights. 
% \systemname features a three-level progressive analysis workflow: starting with a segregation overview, delving into the detailed factors that drive it in Census Block Groups (CBGs) with intervention potential, and ending with formulating and evaluating interventions to mitigate segregation.
% In addition, a series of coordinated visualization views are proposed to assist users throughout the analysis workflow: a Community View with community signatures for demographic comparison, a CBG View for in-depth analysis of CBGs, integrated with a metaphor-based Map View for understanding neighborhood interactions, and a What-If View for evaluating intervention strategies.
% Through case studies and expert interviews, we validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive and equitable environments.
% }

%% Abstract section.
% V0
% \abstract{%
% Segregation is a severe social problem today that hampers community integration and diversity, isolating a city into different filter bubbles. This makes understanding and mitigating segregation a vital goal for social science researchers and policymakers.
% Recently, the availability of large-scale human mobility data has provided new opportunities to measure more fine-grained segregation in activity space.
% However, there lacks an efficient visual analytics approach for in-depth analysis of segregation and formulation of feedback-driven intervention strategies. 
% In this study, we address this gap by introducing \systemname, an interactive visual analytics system designed to empower social scientists to understand mobility-based urban segregation and develop effective urban planning interventions. 
% \systemname features a comprehensive three-level analysis workflow, allowing for an initial exploration of overall segregation, followed by an in-depth examination of the factors driving it, and concluding with the formulation and assessment of intervention strategies.
% In addition, a series of coordinated visualizations are proposed, including a Community View with unique community signatures for efficient demographic comparison, a CBG View coupled with metaphor-based Map View to reveal environmental influences on the segregation in a specific CBG and its interactions between neighboring areas, and a What-If View to enable interactive exploration and assessment of various intervention strategies.
% Through case studies and expert interviews, we validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive and equitable environments.
% }

==> archive/sections_for_pvis25_first_sub/01_introduction.tex <==
\section{Introduction}

Imagine invisible lines, not physical walls, dividing a city; residents are segregated based on their wealth, race, and political beliefs. People live in bubbles and rarely interact with those from different sociodemographic backgrounds.
This form of division, known as \textbf{urban segregation}, transcends geography and reinforces social inequalities.
% Such division is known as \textbf{urban segregation}~\cite{white1986segregation}, not by a geographical split, and reinforces social inequalities. 
% It acts as a barrier to resources and opportunities for those from vulnerable groups and hinders the collective inclusivity and vibrancy of our societies. 
To reshape cities into more inclusive and equitable spaces, social scientists and policymakers have increasingly turned their focus to understanding these complex and invisible barriers and attempting to propose actionable interventions to dismantle these divisions~\cite {chetty2020income, nilforoshan2023human}.

Traditionally, research on urban segregation has concentrated on residential areas, utilizing census statistics such as racial composition to analyze segregation patterns within a city~\cite{white1986segregation}.
% The study about urban segregation in social science has primarily focused on the residential areas~\cite{white1986segregation} and applied census statistics (e.g., racial composition) to understand the segregation patterns within a city. 
While informative, this approach provides a relatively narrow lens that only focuses on residential environments. 
It overlooks the full picture of daily activities beyond residential areas, such as workplaces and social venues, potentially biasing the analysis. 
The recent availability of GPS-based human mobility data is broadening segregation studies from ``residential space'' to ``activity space''~\cite{cagney2020urban},  offering a more comprehensive view of how people experience segregation in their daily routine~\cite{wong2011measuring, browning2017socioeconomic, zhang2023human}. 
For instance, researchers try to explain the motivations behind mobility segregation by indexing the segregation and modeling the human daily activity trajectories~\cite{moro2021mobility} and suggest urban planning interventions to bridge 
% diverse 
\dyu{segregated} communities~\cite{nilforoshan2023human}.

However, existing GPS-based approaches primarily rely on data aggregation to offer a general overview of urban segregation, falling short in capturing detailed patterns of local interactions between neighborhoods at a finer scale.
Moreover, these methods lack \textit{data-informed} tools to guide decision-making and \textit{feedback-driven} processes to adjust strategies, making it difficult for social scientists and policymakers to evaluate urban planning interventions effectively. 
% While \yy{GPS-based segregation statistics rely on aggregation} to provide broader insights, they fall short of capturing the intricate local dynamics of segregation and the complex interactions between different spatial units. Moreover, the absence of both a \textit{data-informed} and \textit{feedback-driven} approach makes it difficult for social scientists and policymakers to precisely evaluate and refine intervention strategies. 
% Visual analytics (VA) emerges as a crucial approach to overcome the aforementioned limitations through intuitive visual representations in different levels of detail and interactive interfaces that support trial and error. Nevertheless, designing an effective VA system to bridge the current research gap is non-trivial. 
\dyu{Visual analytics (VA) is an ideal approach to overcome these limitations, but designing an effective VA system in this context is challenging.}

First, a city's mobility dataset typically comprises thousands of spatial units with potential flows---movements of people between different locations---between any two.
Aggregation techniques help grasp overall mobility networks~\cite{von2015mobilitygraphs, zhou2018visual, liu2019tpflow}, but deriving actionable, fine-grained insights for local urban planning remains a significant challenge.
Several VA systems have shown similar promise in urban planning contexts, such as optimizing location choices~\cite{liu2016smartadp, chen2023fslens} or enhancing bus network efficiency~\cite{weng2020towards}. However, they are not tailored for segregation analysis, which requires navigating the socio-spatial complexities of segregation. 
Second, understanding the intricate correlations between environmental features and mobility patterns is essential for designing effective interventions against segregation. 
These correlations are often nonlinear, multifaceted, and vary across regions~\cite{athey2021estimating}. 
Existing systems can \yy{effectively visualize the mobility flows between areas~\cite{adrienko2010spatial, andrienko2016revealing}} or examine environmental impacts within specific regions~\cite{lei2023geoexplainer, yu2023neighviz}\yy{, but they cannot predict or explain mobility flows in relation to segregation patterns.}

To address the above challenges, \dyu{we propose \systemname, a visual analytics system designed to understand urban segregation using mobility data, effectively meeting the complex demands of segregation analysis.}
\yy{
First, to support fine-grained analysis of segregation patterns, we introduce a three-level analysis workflow that guides users from citywide overview to neighborhood-specific insights. 
We further designed metaphor-based bubble glyphs in a Dorling layout to help users efficiently interpret interactions between neighborhoods.
Second, to unravel intricate correlations between environmental features and mobility patterns, we developed a deep learning model based on Deep Gravity~\cite{simini2021deep} to predict mobility flows using these features. The model is equipped with feature impact visualizations, providing instance-level interpretations by showing the contribution of each feature to visitor flows from different social groups.
Finally, to bridge insights and action, \systemname features a dynamic what-if functionality leveraging the deep learning model, allowing users to test urban planning interventions and receive immediate feedback on their effects on segregation patterns.
}


% In particular, we develop a deep learning model based on Deep Gravity~\cite{simini2021deep} to predict mobility flows using environmental features \wyf{for what purpose?}. 
% \yy{
% Furthermore, to explain the nonlinear and group-specific effects of features on mobility patterns, we employ SHAP values~\cite{lundberg2017unified}, which offer a detailed, instance-level interpretation by showing the contribution of each feature to visitor flows from different social groups.
% }
% Leveraging our deep learning model, \systemname further offers a dynamic what-if functionality, enabling users to interactively adjust urban planning parameters, such as modifying community facilities, and observe real-time feedback across the system. This empowers users to test potential interventions and immediately evaluate their effects on segregation patterns, facilitating informed decision-making.

In summary, the main contributions of this work are as follows:
\begin{itemize}[topsep=0pt, itemsep=0.1pt]
% \begin{itemize}[noitemsep, leftmargin=*]
    \item
    We systematically delineate the problem domain for understanding and mitigating urban segregation using mobility data and present three levels of socio-spatial analysis.
    
    \item 
    We introduce a comprehensive data analysis pipeline that supports mobility-based community detection, segregation calculation, mobility flow prediction, and feature impact explanations. The pipeline also supports what-if analyses, laying the groundwork for guiding precise urban planning interventions.
    
    \item 
    We develop \systemname, a visual analytics system with novel visualization designs, such as metaphor-based bubble glyphs, enabling interactive exploratory analysis of segregation patterns and the testing and evaluation of potential urban planning interventions.

    \item 
    % \dyu{Evaluation: case studies} 
    We evaluate \systemname with two case studies and interviews with domain experts to show the system's effectiveness and usability. 
\end{itemize}


==> archive/sections_for_pvis25_first_sub/02_related_works.tex <==
\section{Related Works}

\subsection{Segregation Analysis in Mobility Data}
\label{sec:related_segregation}
% Understanding the segregation pattern in human mobility is crucial for designing inclusive cities that promote equitable access to resources and opportunities. 
Two approaches are typically applied by social scientists to analyze segregation in mobility data: (1) the index-based approach, which measures the segregation level, and (2) the model-based approach, which uncovers underlying reasons for the segregation.

\textbf{Segregation index} 
is a straightforward approach as an indicator of understanding the segregation level in human mobility data.
The index is usually computed based on the demographics of the group of people who visit a place during a period of time. 
The computation formula of the segregation index is diverse, which can be information entropy~\cite{huang2022unfolding}, isolation index~\cite{white1986segregation, athey2021estimating}, or just distribution unevenness~\cite{zhang2023human, moro2021mobility}. 
Depending on the research topic, the main subject of the segregation can involve different attributes, including income, partisan~\cite{zhang2023human}, race~\cite{athey2021estimating}, or a combination of them~\cite{huang2022unfolding}.
However, the segregation index, being merely an aggregated descriptive metric, does not explain the underlying reasons for the segregation patterns in mobility data.

\textbf{Mobility models} offer researchers a detailed examination of the features influencing mobility and segregation patterns.
A classic model is Exploration and Preferential Return (EPR)~\cite{song2010modelling, pappalardo2015returners}, which uses two key parameters, exploration (visiting new places) and preferential return (revisiting previously visited locations), to model the dynamics of human movement trajectories.
Moro \et~\cite{moro2021mobility} extend the EPR by adding a parameter that quantifies an individual motivation to visit new places where their income group is in the minority. 
Nevertheless, modeling complex human behaviors with few parameters may oversimplify the complexity of mobility patterns and their driving factors.
More sophisticated models, like Deep Gravity~\cite{simini2021deep}, utilize a comprehensive set of features—including facility density and demographic information—and employ deep neural networks to predict mobility flow probabilities between locations.
Despite their predictive power, the complexity of neural networks trained on extensive datasets can obscure the key features influencing segregation patterns, making it challenging to derive actionable insights for mitigating segregation.

We propose a data analysis pipeline that computes the segregation indices and models the impact of environmental features on mobility using an adapted Deep Gravity model, with additional support for feature impact explanations and what-if analyses.


\subsection{Human Mobility Visualization}
Human mobility analysis has been widely studied in the visualization community~\cite{deng2023survey}. 
Here, we mainly discuss the most relevant literature about mobility data visualization and mobility model visualization.

\textbf{Mobility data visualization} often uses origin-destination (OD) flow map~\cite{guo2014origin} to visualize an individual’s movement trajectories.
However, OD flow maps can become visually cluttered with dense data. To address this, researchers have developed alternative visualization techniques such as matrix representations, where each cell indicates flow volume while preserving spatial layout~\cite{wood2010visualisation, yang2016many}. 
Additionally, techniques leveraging data mining, including clustering~\cite{von2015mobilitygraphs, liu2019tpflow, shi2020urbanmotion} and Word2Vec~\cite{zhou2018visual}, have been employed to aggregate mobility data and distill key insights, thereby enhancing visualization clarity and interpretability.
Other mobility visualization work further incorporates semantic information, such as point of interest (POI) information~\cite{zeng2017visualizing} and social media text~\cite{chen2015interactive, krueger2019bird}, enriching the contextual understanding of mobility patterns.
However, a notable gap in the literature is the insufficient integration of demographic data into mobility visualization, which is essential for understanding underlying social dynamics such as income and racial inequality~\cite{athey2021estimating, moro2021mobility} and partisan polarization~\cite{zhang2023human}.

\textbf{Mobility model visualization}, primarily studied in the transportation domain, can facilitate understanding the driving factors of mobility patterns.
For instance, visualizing congestion predictions generated by deep learning models can assist experts in analyzing and predicting congestion scenarios~\cite{lee2019visual} and even refining the models~\cite{jin2022visual}.
Meanwhile, TCEVis~\cite{dong2023tcevis} employs SHAP values to offer explainable insights into the features influencing traffic congestion.
However, these models typically focus on entire populations without considering variations across social groups.

Our work not only visualizes the mobility patterns of diverse social groups but also incorporates these distinctions into mobility modeling. 
This approach allows for a visual comparison of the factors driving segregation among different social groups, enhancing the understanding of mobility dynamics within a sociodemographic context.

\subsection{What-If Analysis}
What-if analysis empowers users to explore the predictive models by adjusting input features, thereby understanding the model's behavior under various hypothetical scenarios.
Visual analytics systems enhance this exploration by facilitating interactive feature adjustments to observe their impact on predictions~\cite{krause2016interacting, wexler2019if, cheng2021vbridge}.
In the urban planning scenario, what-if analysis is widely embedded in many planning support systems, such as $\rm{What-If?}^{TM}$~\cite{klosterman2008whatif} and CommunityViz~\cite{janes2008communityviz}, as well as traffic analysis systems~\cite{andrienko2016leveraging} and public policy simulators~\cite{yang2022epimob, usman2022multiscale}. 
These systems facilitate data-driven decision-making by enabling stakeholders to simulate and evaluate the consequences of various urban design scenarios. 
However, a common limitation among these tools is their lack of focus on the goal of promoting inclusivity through urban planning.
CityScope~\cite{alonso2018cityscope} more closely aligns with our objectives by offering a tangible interface that promotes urban performance metrics, including the exposure diversity of different social groups.
Nevertheless, the agent-based modeling behind CityScope, relying on parameters distilled from surveys or regression~\cite{grignard2018impact}, may oversimplify the diverse social and environmental nuances of urban settings.

Our approach addresses these limitations by developing a deep learning model that not only captures complex correlations between environmental features and segregation but enables a what-if analysis to provide real-time feedback on the effectiveness of user-defined interventions for segregation mitigation. We further presented a set of tailored visualizations based on superposition approaches to support comparative analysis between different intervention strategies.

==> archive/sections_for_pvis25_first_sub/03_background.tex <==
\section{Background}

% In this section, we first introduce the analytical goals distilled together with the expert, which derive five visualization design tasks. We then introduce the system overview.

\subsection{Requirement Analysis}
\label{prob_formulation}
\label{sec:03_Background_VisualizationDesignTasks} 

Over the past year, during the design phase of our system, we closely collaborated with social scientist $E_A$ to shape the design of \systemname.
$E_A$ is an experienced sociologist in using human mobility data for urban segregation analysis with a number of relevant publications focusing on the causes and mitigation of partisan segregation. 
During the evaluation phase, we also involved experts $E_B$, $E_C$, and $E_D$, \yy{all with a focus on segregation but from diverse backgrounds} (detailed in Section~\ref{sec:evaluation}).
Through monthly discussions with $E_A$ and extensive literature reviews, we found that traditional urban segregation studies mainly focus on designing segregation indices and using regression analyses to associate environmental features with segregation levels~\cite{zhang2023human, huang2022unfolding, athey2021estimating}.

These methods offer an overview of segregation patterns, but examining detailed local mobility dynamics and the interactions between spatial units often requires labor-intensive, ad-hoc analysis, which can be time-consuming.
To address these limitations, we have first identified two primary analysis goals, \textit{Community-level Analysis} and \textit{Census Block Group (CBG)-level Analysis}, to facilitate a comprehensive exploration and analysis of segregation patterns \yy{from community-level overview to detailed local dynamics among different social groups.}
In our study, a CBG is a basic and precisely defined spatial unit with 600-3000 residents; a community consists of multiple CBGs, resembling a larger district within a city.
\yy{``Social group'' refers to distinct categories of individuals sharing common characteristics, such as income, race, partisan affiliation, or other demographic attributes.}
%, where people tend to interact more frequently within those areas.


During our discussions, $E_A$ expressed keen interest in identifying strategic urban planning methods to counteract the observed segregation, alongside a straightforward approach to assess the impact of proposed plans.
Though there are tools for simulating the effects of urban policies~\cite{klosterman2008whatif, janes2008communityviz, alonso2018cityscope}, he noted they lack integration with segregation analysis, making it challenging to assess the social impacts of urban planning.
Also, among various urban planning interventions, $E_A$ suggested adjusting different types of Points of Interest (POIs) as a practical strategy for addressing segregation.
Consequently, we identified the third goal: \textit{Point of Interest (POI)-level Analysis}, to allow for interactive exploration and assessment of POI modifications to promote inclusivity.
Overall, we have summarized the following three-level socio-spatial analysis goals.

% \textbf{\commpill unity-level Analysis.} The expert aims to obtain an overview of the city's segregation dynamics at a community level, which is a great information granularity for identifying a focus area for detailed analysis. 
% This involves examining the mobility patterns and sociodemographic characteristics of communities.
\textbf{\commpill unity-level Analysis} enables experts to obtain an overview of the city’s segregation dynamics at the community level. This granularity helps identify focus areas for detailed analysis by examining mobility patterns and sociodemographic characteristics of communities.

% \textbf{\cbgpill-level Analysis.} Within the focus community, the expert wants to identify specific CBGs that could serve as pilot areas for mitigating segregation. 
% Therefore, the system should facilitate the efficient identification of these CBGs that present opportunities for intervention and the exploration of how their features affect the movement of people from different social groups.

\textbf{\cbgpill-level Analysis} facilitates the identification of specific CBGs that could serve as pilot areas for mitigating segregation within selected communities. This involves efficiently pinpointing CBGs with significant segregation but intervention potential and exploring how their features influence the movement of people from different social groups.

% \textbf{\poipill-level Analysis.} Given a selected CBG, the expert aims to adjust POIs within this CBG to reduce segregation and promote inclusivity.
% Thus, the system should allow for comparing the effectiveness of different POI adjustments in promoting inclusivity. 
% The expert wants to explore and compare the effectiveness of different POI adjustments in promoting inclusivity.

\textbf{\poipill-level Analysis} allows experts to adjust POIs within selected CBGs to reduce segregation and promote inclusivity. This involves comparing the effectiveness of different POI modifications in fostering inclusive environments.

We have further identified five design requirements to support the three-level socio-spatial analysis goals: 
% In light of the goals above, we have then collaborated with $E_A$ through iterative interviews, and subsequently, we derived five visual analysis tasks to support the three-level socio-spatial analysis above:

\hangpara{2em}{1}
\TIpill{} \textbf{Segment and characterize communities.} 
The system should identify communities based on human mobility and characterize them by the demographics of population flows, enabling the expert to understand how populations move between communities and how citywide segregation is shaped by these flows.
% to help the expert understand how they are interconnected. 

\hangpara{2em}{1}
\TIIpill{} \textbf{Compare sociodemographics across communities.} 
The system should support a comparative analysis of sociodemographic attributes across communities, including both residents and visitors. 
This will enable the expert to detect communities where segregation in activity spaces is prominent, guiding further investigation.
% to help the expert identify a community exhibiting significant segregation in activity space for further investigation.

\hangpara{2em}{1}
\TIIIpill{} \textbf{Identify CBGs with intervention potential.} 
Within a selected community, the system should assist the expert in identifying CBGs that show significant segregation levels and high potential for effective interventions. 
A multi-criteria ranking of segregation-related metrics of all CBGs within this community is thus necessary to prioritize areas for targeted action. 
% Within a selected community, the system should list the CBGs ranked by multiple segregation-related criteria.
% This will assist the expert in pinpointing CBGs that show significant segregation levels and have a high potential for effective interventions. 

\hangpara{2em}{1}
\TIVpill{} \textbf{Analyze target CBG inflow and influential features.} 
Once a target CBG is selected, the system should provide a detailed analysis of the inflow patterns across social groups and illustrate how key environmental features influence these patterns.
This will help the expert identify factors contributing to segregation. 
By distinguishing how each group responds to these features, the expert can better assess if certain groups are excluded or isolated, offering deeper insights into segregation dynamics.

\hangpara{2em}{1}
\TVpill{} \textbf{Simulate urban planning interventions.} 
To facilitate practical applications, the system should support the expert in conducting ``what-if'' analyses by modifying POI features in the target CBG to reduce segregation.
This requires simulating and visualizing the real-time impact of these changes on mobility patterns and segregation levels, supporting the expert to access the practical interventions for promoting inclusivity.

\begin{figure} []
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/system overview_v2.png}
 \vspace{-0.5cm}
 \caption{
    System overview - \systemname comprises three modules: Data, Analysis Pipeline, and Visualization, to support interactive segregation analysis (\commpill{} and \cbgpill) and iterative intervention development (\poipill).
 } 
 \vspace{-0.4cm}
 \label{fig:system-overview}
\end{figure}

\subsection{System Overview}
\label{sec:system-overview} 
To address the identified requirements, we developed \systemname, an open-source human-in-the-loop VA system\footnote{\url{https://anonymous.4open.science/r/inclusiviz/}} consisting of three modules (Fig.~\ref{fig:system-overview}).
The Data module stores data in a database in the structures as detailed in Section \ref{sec:data_abstraction}.
The Analysis Pipeline module integrates mobility-based community detection (Section \ref{sec:community_detection}), segregation measures (Section \ref{sec:segregation_measures}), and a deep learning model (Section \ref{sec:model}) enhanced with explainable AI techniques that pinpoint influential features (Section \ref{sec:model_shap}) and evaluate the impact of user-defined urban planning interventions (Section \ref{sec:model_what_if}).
\yy{
Importantly, the pipeline is designed to be flexible and model-agnostic. Both the model and explainable AI techniques can be easily updated or replaced, ensuring compatibility with newer models or methods in the domain.
}
Finally, the Visualization module consists of four coordinated views (Section \ref{sec:05_visual_design}), allowing users to explore analysis results and experiment with hypothetical interventions.
%, and receive real-time feedback on potential outcomes.



==> archive/sections_for_pvis25_first_sub/04_data_analysis.tex <==
\section{Data Analysis Pipeline}
\label{sec:04_Data_Analysis}
This section outlines the data abstraction and the components of our analysis pipeline, which are designed to analyze segregation patterns and model mobility data effectively.

\subsection{Data Abstraction}
\label{sec:data_abstraction}
We have collected three datasets for the same city in the U.S.
We use the Census Block Group (CBG) as the basic spatial unit, a detailed division frequently used in social science research that uses U.S. data. According to the U.S. census, each CBG typically encompasses 600 to 3000 residents. 
This choice of unit ensures fine-grained analysis, but our system is adaptable to other spatial divisions, such as England's Lower Layer Super Output Areas (LSOA). 
Below is a description of each dataset:

\begin{itemize}[topsep=0pt, itemsep=0.2pt, leftmargin=*]
    \item \textit{Mobility Dataset} contains the aggregated movement of individuals between various CBGs over one year. 
    It is structured as a directed weighted graph $ G = (V, E) $, where each node $ v \in V $ is a CBG, and each edge $ (v_i, v_j) \in E $ represents the flow of individuals from CBG $ v_i $ to $ v_j $, weighted by the count of these individuals, $ w(v_i, v_j) $.
    In our study, we utilized data provided by $E_A$, aggregated from SafeGraph. 
    This dataset encompasses large-scale monthly mobility flows from origin CBGs to destination places, collected from anonymous mobile devices, covering approximately 10\% of the entire U.S. population.
    
    \item \textit{Sociodemographic Dataset} contains population characteristics of each CBG (\eg, income and race)
    For an attribute $ D $ (\eg, income level), it has a matrix $ S_D = [s_{id}] $, where $ s_{id} $ is the population count of a social group $ d \in D $ (\eg, \$ 50K-100K income group) of CBG $i$.
    We obtained the data from the 5-year American Community Survey and L2 Political Academic Voter File.
    
    \item \textit{POI Dataset} contains the density (number per square kilometer) of each type of POI in each CBG. 
    It is formatted as a matrix $ P = [p_{ip}] $, where $ p_{ip} $ represents the density of POI type $ p $ in CBG $ i $.
    In our study, this dataset is also sourced from SafeGraph, containing 12 major POI types such as food, shopping, work, health, and others.
\end{itemize}

\begin{figure}
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/data_v2.png}
 \vspace{-0.5cm}
 \caption{
    In the data analysis pipeline, the Segregation Measures (A) computes each CBG's Segregation Index (1) and Bridging Index (2), and then ranks them using Dual-Attribute Ranking (3).
    The Mobility Data Modeling (B) trains a Deep Learning Model for a social group (1), enhanced with \yy{Feature Impact} (2) and What-If Analysis (3) modules.
    % (A) The computation of two segregation measures: 1. segregation index and 2. bridging index.
    % (B) Mobility Data Modeling, consisting of 1. a Deep Gravity Model for each social group, 2. a Partial Dependence Plots module, and 3. a What-If Analysis module.
 }
 \vspace{-0.4cm}
 \label{fig:data_analysis}
\end{figure}

\subsection{Mobility-based Community Detection}
\label{sec:community_detection}

In segregation studies, clustering spatial units in a city into communities with high internal movement but limited external interactions can effectively reveal data-driven social boundaries, offering a clear overview of segregated areas~\cite{huang2022unfolding, burdick2020socially} \yy{(\TIpill)}.

For community detection in directed weighted graphs that align with our \textit{Mobility Dataset}, multiple community detection algorithms are available, including flow-based InfoMap~\cite{rosvall2009map} and modularity-based Leiden~\cite{traag2019louvain}.
These algorithms offer distinct advantages: the Leiden algorithm tends to segment larger community structures, while the InfoMap algorithm tends to identify sub-communities~\cite{gibbs2021detecting}. 
Considering our objective of maintaining a manageable number of communities for an interpretable overview as the initial analysis, we adopt the Leiden algorithm.
The algorithm takes an edge list, where each entry contains the source CBG $v_i$, the destination CBG $v_j$, and the flow weight $w(v_i, v_j)$, as input and iteratively optimizes modularity by reassigning CBGs to communities.
% The Leiden algorithm initially assigns every CBG as an independent community. Then, the algorithm iteratively moves CBGs between communities to enhance the overall modularity.
% After achieving local optimality, it combines CBGs in communities and rebuilds the network, and repeats. The algorithm concludes when there's no further improvement in modularity.
To focus on significant mobility patterns, we apply a customizable flow threshold $w_{min}$ to retain only edges where $w(v_i, v_j) \geq w_{min}$.
For interpretability, we focus on the 10 largest communities, grouping the remaining CBGs into an ``others'' category.


\subsection{Segregation Measures}
\label{sec:segregation_measures}
\dyu{We employ the Segregation Index and the Bridging Index to quantify and prioritize segregation patterns. We also implement Dual-Attribute Ranking method to prioritize CBGs for intervention.}

\subsubsection{Segregation Index}
\label{sec:segregation_index}
The segregation index (Fig.~\ref{fig:data_analysis}-A-1) is a common practice to quantify the segregation level of visitors in an area \yy{(\TIIpill)}.
Different formulas have been developed for the segregation index using mobility data as discussed in Section \ref{sec:related_segregation}.
In this study, we adopt the distribution unevenness recommended by our expert due to its ease of interpretation~\cite{zhang2023human}.

For any target CBG $v_{target}$ visited by $N$ source CBGs, to calculate its segregation index of a sociodemographic attribute $D$, we first determine the proportion of residents in each social group $d$ in each source CBG $v_i$ as $\theta_{id}$. 
Next, for each social group $d$, we calculate the proportion of visitors from $d$, $\pi_d$, using the equation:

\begin{equation}
\label{equation:segregation_prop}
    \pi_d(v_{target}) = \sum_{i=1}^{N} \frac{\theta_{id} \times w(v_i, v_{target})}{\sum_{i=1}^{N} w(v_i, v_{target})}
\end{equation}

Finally, the segregation index ($SI_D$) is computed using the equation below, normalized to range between 0 and 1 by the factor $\frac{n}{2n-2}$ (higher values indicate greater segregation):

\begin{equation}
\label{equation:segregation_index}
    SI_D(v_{target}) = \frac{n}{2n-2} \times \sum_{d \in D} \left| \pi_d(v_{target}) - \frac{1}{n} \right|
\end{equation}

\subsubsection{Bridging Index}
While traditional segregation indices highlight divisions, the bridging index (Fig.~\ref{fig:data_analysis}-A-2), proposed in~\cite{nilforoshan2023human} emphasizes opportunities for integration and connection.
It can identify possible ``bridges'' for social integration by computing the diversity of social groups interacting in a hub, assuming everyone visits their nearest hub.
However, due to limitations in our dataset, we adapt this concept by treating a CBG as a hub and focusing on the $k$ nearest CBGs to each $v_{target}$, where $k$ is adjustable. 
We first estimate the proportion of residents from each group $d$ within these CBGs who might visit $v_{target}$, where $p(v_i)$ is the population size of a source CBG $i$:

\begin{equation}
    \pi_d(v_{target})\prime = \sum_{i=1}^{k} \frac{\theta_{id} \times p(v_i)}{\sum_{i=1}^{k} p(v_i)}
\end{equation}

Then, we measure the bridging index ($BI_D$),  using the following equation, which is the inverse of the segregation index:

\begin{equation}
\label{equation:bridging_index}
    BI_D(v_{target}) = 1 - \frac{n}{2n-2} \times \sum_{d \in D} \left| \pi_d(v_{target})\prime - \frac{1}{n} \right|
\end{equation}

\begin{figure*} [t!]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/system_v2.png}
 \vspace{-0.5cm}
 \caption{
     The interface of \systemname guides experts through a segregation analysis and iterative intervention design workflow. 
     In the \commview (A), experts analyze the sociodemographic profiles and interconnections of mobility-based communities, identifying areas with potential segregation.
     Experts then drill down into the \cbgview (B) to select a target CBG for intervention, investigating how its features influence inflow patterns from different social groups.
     Meanwhile, the \mapview (C) offers geographic context for these mobility patterns.
     Finally, experts use the \whatifview (D) to simulate urban planning interventions, with the predicted impact of those changes reflected directly in the \cbgview (B) and the \mapview (C).
 }
 \vspace{-0.4cm}
 \label{fig:system-visual}
\end{figure*}

\subsubsection{Dual-Attribute Ranking}
\label{sec:TOPSIS_ranking}
Research by Nilforoshan \et~\cite{nilforoshan2023human} highlights a strong inverse relationship between bridging and segregation indices.
While relocating residents to bridge different social groups is beneficial, it is too ethically complex and thus impractical for our study~\cite{sanbonmatsu2011moving}. 
In consultation with our expert, we shifted focus towards CBGs with high bridging index (diverse neighborhoods) yet still experiencing high segregation.
These offer the potential for interventions to increase visitor diversity \yy{(\TIIIpill)}.

A Multi-Criteria Decision Making (MCDM) method can help us more easily prioritize the CBGs with both high segregation index $SI$ and bridging index $BI$.
% This approach is crucial for prioritizing CBGs for intervention and for organizing them in the \cbgTable discussed in Section~\ref{vis:cbg_view}. 
Among various MCDM techniques, we selected the Technique for Order of Preference by Similarity to the Ideal Solution (TOPSIS)~\cite{lai1994topsis} for its simplicity and effectiveness.
TOPSIS ranks CBGs based on their proximity to both ideal (high $BI$ and $SI$) and negative-ideal (low $BI$ and $SI$) benchmarks (Fig.~\ref{fig:data_analysis}-A-3). 
It effectively surfaces CBGs that not only are positioned well for fostering integration but also currently suffer from high segregation.

\subsection{Mobility Data Modeling}

\subsubsection{Deep Learning Model}
\label{sec:model}
We developed a deep learning model adapted from Deep Gravity~\cite{simini2021deep} (Fig.~\ref{fig:data_analysis}-B-1), the state-of-the-art deep learning framework designed to predict mobility flows based on environmental features including distance, population size, land use, and densities of different types of POI.
We made two key adaptations for segregation analysis, which, as evaluated in Section~\ref{sec:model_evaluation}, improved the model's prediction precision.

\begin{itemize}
    \item Social group segmentation: 
        We divide the \textit{Mobility Dataset} ($G$) into segments ($G_d$) for each social group $d \in D$, enabling separate models to capture group-specific mobility patterns.
    \item Visitor characteristics inclusion:
        Inspired by Moro \et~\cite{moro2021mobility} that models the preference of people to visit the places where they are the minority in visitors, we include the sociodemographic characteristics of visitors computed using Equation \ref{equation:segregation_prop} as part of the input vectors. 
        This aims to model how different social groups respond to the visitor characteristics of a destination area.
\end{itemize}

Our adapted model's input for an origin-destination CBG pair $(v_i, v_j)$ is $concat[p_i, p_j, x_i, x_j, \pi_j, dis_{i,j}]$, where $p_i$, $p_j$ are the population sizes, $x_i$, $x_j$ represent densities of different types of POIs of the origin and destination, $\pi_j$ is a vector for the visitor characteristics of the destination, and $dis_{i,j}$ is their geographical distance. 
We employ a neural network architecture consistent with the original Deep Gravity model consisting of 15 hidden layers, combining wider layers (256 neurons) and narrower layers (128 neurons) with LeakyReLU activations.
The network predicts a mobility likelihood score $s(v_i, v_j)$ for each origin-destination CBG pair. For each origin CBG $v_i$, it calculates these scores for $k$ randomly selected destinations, and here $k$ is set to be 30 to speed up the computation.
The likelihood scores are transformed into predicted probabilities using the softmax function, and the predicted flow volume from $v_i$ to $v_j$, $\hat{w}(v_i, v_j)$, is calculated by multiplying the total number of individuals from $v_i$ to its $k$ destinations with its probability:

\begin{equation}
    \hat{w}(v_i, v_j) = \left( \sum_{l=1}^{k} w(v_i, v_l) \right) \cdot \frac{e^{s(v_i, v_j)}}{\sum_{l=1}^{k} e^{s(v_i, v_l)}}
\end{equation}

\subsubsection{\yy{Feature Impact}}
\label{sec:model_shap}
\yy{
To understand how individual features influence predictions in our deep learning model \yy{(\TIVpill)}, we utilize SHAP values~\cite{lundberg2017unified} (Fig.~\ref{fig:data_analysis}-B-2), a widely adopted explainable AI technique.
SHAP quantifies each feature's contribution to the predicted likelihood of mobility flows, capturing both the direction and magnitude of its influence.
Unlike Partial Dependence Plots (PDP), which show only average effects, SHAP provides more granular, instance-specific insights. 
We chose SHAP over other local explanation techniques like LIME~\cite{ribeiro2016should} for its basis in Shapley values, ensuring fair and consistent feature attribution across instances for more stable explanations.
}

\yy{
We use \texttt{DeepExplainer} module from the SHAP library, which is well-suited for approximating feature contributions within deep neural networks.
For each social group's model, SHAP values of the features are computed for the predicted flow $\hat{w}(v_i, v_{target})$ between a pair of origin and target CBG $(v_i, v_{target})$. 
For efficiency, we precompute 50 centroids via K-means clustering as the background dataset for the SHAP explainer, ensuring representative feature impact approximations.
}

\subsubsection{What-If Analysis}
\label{sec:model_what_if}
To allow users to explore the potential impact of hypothetical urban planning changes on mobility patterns \yy{(\TVpill)}, we developed a What-If Analysis module to enhance the deep learning model (Fig.~\ref{fig:data_analysis}-B-3).
When some POI-related features in the target CBG ($v_{target}$) are modified as $x_{target}\prime$, the function modifies the input vector for each pair of origin and target CBG $(v_i, v_{target})$, resulting in a new set of input vectors $concat[p_i, p_{target}, x_i, x_{target}\prime, \pi_{target}, dis_{i, {target}}]$.
These modified vectors are then fed to our trained models to predict new mobility flows \(\hat{w}_{after}(v_i, v_{target})\) from different social groups.
To quantify the impact of the change, we calculate the difference between the predicted flows before and after the hypothetical intervention using the equation below, and increment the predicted differences to actual flow volumes accordingly, as the new flow volumes resulting from feature adjustments:

\vspace{-0.5cm}
\begin{equation}
    \Delta \hat{w}(v_i, v_{target}) = \hat{w}_{after}(v_i, v_{target}) - \hat{w}_{before}(v_i, v_{target})
\end{equation}

==> archive/sections_for_pvis25_first_sub/05_visual_design.tex <==
\section{Visual Design}
\label{sec:05_visual_design}

\systemname consists of four views to fulfill the analysis goals introduced in Section~\ref{sec:03_Background_VisualizationDesignTasks}: \commview (Fig.~\ref{fig:system-visual}-A), \cbgview (Fig.~\ref{fig:system-visual}-B), \mapview (Fig.~\ref{fig:system-visual}-C), and \whatifview (Fig.~\ref{fig:system-visual}-D).
We demonstrate the seamless analysis flow using the four views with an illustrative use case derived:
A social scientist investigates income-based segregation in a city.
After analyzing the interconnection between detected mobility-based communities (\TIpill) and comparing their sociodemographic distributions (\TIIpill) in the \commview, he notices one with a significant low-income concentration, indicating segregation.
Drilling down into this community in the \cbgview, he identifies a target CBG with high segregation and potential for intervention (\TIIIpill).
Cross-referencing inflow patterns of the target CBG in the \mapview with \yy{the feature impact in the \whatifview}, he observes a lack of health-related POIs in the target CBG, which could explain its limited appeal to higher-income groups (\TIVpill).
Finally, using the \whatifview to simulate an increase in such POIs, he receives feedback suggesting this intervention could reduce segregation (\TVpill).
% After identifying a segregated community of interest, \cbgview (Fig.~\ref{fig:system-visual}-B) helps pinpoint CBGs with potential for intervention (\TIIIpill).
% Meanwhile, \mapview (Fig.~\ref{fig:system-visual}-C) and \cbgview work together to reveal how environmental features influence the inflows of different social groups to the target CBG (\TIVpill).
% Finally, \whatifview empowers experts to simulate urban planning changes and assess their potential impact on segregation (\TVpill), receiving real-time feedback in both \cbgview and \mapview.

\subsection{Community View}
The \commview (Fig.~\ref{fig:system-visual}-A) provides an overview for exploring mobility-based community structures within the city and their sociodemographic characteristics.
It allows experts to customize the city and attribute of interest and the flow threshold, and detect communities using the Leiden algorithm as described in Section~\ref{sec:community_detection}.
Then, it supports the comparison of community sociodemographic profiles using the \commsig (Fig.~\ref{fig:system-visual}-A1) (\TIIpill) and inter-community flows in the \flowmat (Fig.~\ref{fig:system-visual}-A2) (\TIpill).
Finally, experts can indicate a community of interest for the following analysis.

\textbf{\commsig.}
To support the efficient analysis of the sociodemographic profiles of detected communities, a \commsig of each attribute accompanies each community, displayed in its corresponding color (\TIIpill).
The top row features the signatures of the chosen attribute, while subsequent rows provide additional attribute signatures as auxiliary information.
A signature (Fig.~\ref{fig:signature}-A) resembles horizontally aligned boxplots (Fig.~\ref{fig:signature}-B), with only the interquartile range (IQR) preserved and linked by smooth lines.
Within each IQR box in a signature, its height represents the range of proportions for a social group within the central 50\% of CBGs in the community, with the median line highlighted in a darker color for emphasis
A detailed legend about the signatures of an attribute will be shown upon hovering over the question mark icon beside the attribute name.

\textit{Justification:}
We initially displayed distributions using traditional boxplots (Fig.~\ref{fig:signature}-B). 
However, our domain expert found them visually overwhelming when comparing sociodemographic profiles across multiple communities. 
He suggested that at the early analysis stage, social scientists often focus on the distributions within the majority of CBGs in a community to gain an overall impression. 
Therefore, we designed the \commsig to emphasize the essential IQR information, representing the central concentration of CBGs, while simplifying the visual presentation.
Connecting IQRs with lines enhances visual continuity, aiding efficient comparison.
Our expert further recognized that this design streamlined his analysis, allowing him to rapidly identify similarities and differences between community attribute distributions based on the signature shapes.
% We originally adopted a traditional way to display the distributions by boxplots (Fig.~\ref{fig:signature}-B). 
% However, while boxplots offer detailed distribution data, they can become visually overwhelming when used in multiples. 
% After consulting to our domain expert, he mentioned that social scientists may only focus on the distributions of majority CBGs in an large area, 
% The \commsig design retains the essential IQR information and the median value for each social group while streamlining the visual presentation.
% Furthermore, IQRs are connected with lines which enhance visual continuity, facilitating the efficient analysis of community socioeconomic profiles.

\begin{figure} [t]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/design-signature.png}
 \vspace{-0.5cm}
 \caption{
     (A) The income \commsig design to show the income distributions of CBGs in community B. 
     (B) shows an alternative design: traditional boxplots.
     (C) The visual encoding of a cell in the \flowmat.
 }
 \vspace{-0.6cm}
 \label{fig:signature}
\end{figure}

\textbf{\flowmat.}
The \flowmat visualizes inter-community mobility patterns within the city (\TIpill), which has been segmented into N communities.
This $(N+1) \times (N+1)$ matrix resembles the adjacency matrix of a directed weighted graph. 
In the matrix, rows represent community outflows, columns represent inflows, and the final column/row depicts total flows.
Each matrix cell (Fig.~\ref{fig:signature}-C) encodes the visitor flow between two communities, and bars within the cell represent the proportions of different social groups (consistent with the encoding in the \commsig).
A log-normalized scale represents flow volume through the background color of the bars, and the flow volume can be aggregated as mean, median, sum, and standard deviation via the ``Flow aggregation'' selector above. 
Community labels on the left act as selectors for experts to choose a community of interest.

\textit{Justification:}
While a node-link visualization was considered, we adopted the matrix representation to visualize the multivariate flows and their attributes for its effectiveness of matrices for comparing edge attributes~\cite{nobre2019state, alper2013weighted}.
In our case, these attributes represent the crucial distribution of social groups within the flows between communities.

\subsection{CBG View}
\label{vis:cbg_view}
The \cbgview (Fig.~\ref{fig:system-visual}-B) presents a \cbgTable to identify CBGs with intervention potential for mitigating segregation within a chosen community (\TIIIpill).

The interactive \cbgTable inspired by the Ranking View in SmartAdp~\cite{liu2016smartadp} displays a list of CBGs ranked by TOPSIS, as described in Section~\ref{sec:TOPSIS_ranking}, that prioritizes the CBGs in diverse neighborhoods but experiencing high segregation (\TIIIpill).
Each row showcases a CBG with the geographical boundary shape, segregation index $SI$ and bridging index $BI$ (with bars representing their magnitudes), and proportions of social groups behind these two indices (encoded with bar charts consistent with the \flowmat).
Experts can adjust the $k$ neighbors parameter at the top to modify the bridging index calculation and reorder the table.
Selecting a CBG row will set it as the target CBG, allowing detailed feature impact exploration in the \whatifview and inflow pattern analysis in the \mapview.

\subsection{Map View}
\label{vis:map_view}
The \mapview (Fig.~\ref{fig:system-visual}-C) provides geographical information, juxtaposing the \realmap (Fig.~\ref{fig:system-visual}-C1) for geographical context for the detected communities (\TIpill) and the \dorlingmap (Fig.~\ref{fig:system-visual}-C2) to analyze the detailed flows between CBGs (\TIVpill).

\textbf{\realmap}. It displays the city's map with color-coding CBGs according to their community assignment. It offers two modes: ``full mode'' reveals the entire city, while ``focus mode'' highlights a selected target CBG (in black) and its closest $k$ neighbors, where $k$ adjusts based on settings in the \cbgTable of the \cbgview (Section~\ref{vis:cbg_view}).

\textbf{\dorlingmap}. It employs a Dorling layout~\cite{dorling1996area} to preserve relative CBG positions to allow more informative representations of the target CBG and its neighbors by glyph encoding.
Specifically, a \bubbleglyph (Fig.~\ref{fig:system-visual}-C3) visualizes the detailed information of a CBG.

\textbf{\bubbleglyph.}
Inspired by the concept of social filter bubbles that isolate people into homogeneous individuals, we designed the metaphor-based \bubbleglyph to showcase one CBG's resident demographics and flow patterns, as shown in Fig.~\ref{fig:glyph}.
The background color of the glyph matches the CBG's assigned community, and the glyph's radius represents the population size of the CBG.
The CBG's actual geographical boundary shape is at the center inside the glyph to aid in connecting with \realmap and \cbgTable.
A circle of white proportion arcs around the shape represents the proportions of different social groups in the CBG's resident population.
The arcs resemble the reflection light on a bubble: the dominance of one arc will create a bubble-like appearance, visually indicating segregation.
When an arc is hovered, its full axis will show the maximum possible length of the arc, with a tooltip showing the detailed group name and proportion values.
A thicker flow arc around the boundary represents the proportion of residents visiting the target CBG.

\textit{Justification:}
We designed the bubble glyph after carefully considering several alternatives \yy{with our expert} (Fig.~\ref{fig:glyph}-B, C).
\yy{Design B encodes the proportion of outgoing visitors from each CBG to the target CBG by the thickness of a darker inner edge, and represents the proportions of different social groups within that CBG with a pie chart.
However, as the number of glyphs increases on the map, these edges begin to cross over each other, leading to severe visual clutter.}
Design C places social group proportions as a bar chart consistent with \flowmat, which saves space.
However, this layout limits the flow arc to less than a full circle, which is counter-intuitive and potentially misleading for chart reading.
In contrast, the \bubbleglyph remains the expert's favored design as it is intuitive and aesthetically pleasing.
Its metaphor-based approach vividly communicates segregation while avoiding issues like edge crossings, and it facilitates clearer comparisons of demographic proportions across multiple CBGs.


\begin{figure} [t]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/design-glyph_v2.png}
 \vspace{-0.5cm}
 \caption{
     (A) The \bubbleglyph design to demonstrate one CBG's resident sociodemographics and flow patterns to target CBG.
     (B) and (C) show two alternative glyph designs.
 }
 \vspace{-0.6cm}
 \label{fig:glyph}
\end{figure}

\subsection{What-If View}
The \whatifview (Fig.~\ref{fig:system-visual}-D) enables users \yy{to explore how environmental features influence the number of visitors from different social groups to a target CBG (\TIVpill) and} design hypothetical interventions for reducing segregation for the CBG (\TVpill).
\yy{
At the top, a CPC bar (introduced in Section~\ref{sec:model_evaluation}) shows the trained model's predictive accuracy in the target CBG.
Below, it juxtaposes a \featControl (Fig.~\ref{fig:system-visual}-D1) and \featImpacts for different social groups (Fig.~\ref{fig:system-visual}-D2).}

\yy{\textbf{\featControl}. A list of Kernel Density Estimate (KDE) plots depicts the global distributions of features across the entire dataset, with the current values for the target CBG indicated by draggable lines. Users can interactively adjust feature values by dragging these lines horizontally (\TVpill). 
% The adjustments will be dynamically fed into the deep learning model's What-If Analysis module (Section~\ref{sec:model_what_if}), triggering updates across visualization components.
Expert feedback indicates that mitigating segregation is more feasible through adjustments in POI rather than demographic characteristics, so the panel lists only POI-related features by default, with an option to expand the panel to access the full feature list, including both sociodemographic and POI-related factors.
}

\yy{
\textbf{\featImpact}. A \featImpact illustrates how features in the target CBG influence the flow of visitors from a social group in neighboring CBGs (\TIVpill). At the top of each column, the proportion of visitors from the social group is visualized as a bar chart, consistent with the chart in the \cbgview. Below, each feature's average SHAP value is shown as a dot with error bars for standard deviation, indicating the strength of its influence on attracting or repelling visitors from the social group to the target CBG.
By default, features are ordered by the sum of their SHAP value magnitudes. 
Following expert recommendations, the system also allows sorting by the variance in SHAP values across social groups, facilitating inter-group comparisons of mobility behaviors.
% However, based on expert recommendations, the system also allows sorting by the variance in SHAP values across social groups to facilitate inter-group comparisons of mobility behaviors.
For more detailed instance-level explanations, when users hover over a social group arc in the \bubbleglyph of a specific CBG $v_i$, a line connecting the individual SHAP values overlays the dots, illustrating how features in the target CBG $v_{target}$ affect visitor behavior from that social group within $v_i$.
}

\subsection{Providing Real-time Feedback}
\label{vis:interaction}
To enable users to develop and evaluate urban planning interventions with real-time feedback (\TVpill), adjustments made to the target CBG’s features in the \featControl of the \whatifview are dynamically fed into two modules: the deep learning model’s Feature Impact (Section~\ref{sec:model_shap}) and What-If Analysis (Section~\ref{sec:model_what_if}). These modules recalculate the SHAP values for the features and predict new mobility flows from different social groups to the target CBG. Additionally, a new Segregation Index (Section~\ref{sec:segregation_index}) is computed for the target CBG.

This process triggers real-time updates across the visualization components, providing users with immediate feedback for intervention evaluation and refinement. The updates are as follows:

\yy{
\featImpact: Recalculated average SHAP values for the features are displayed as gold dots alongside the original purple dots for comparison (Fig.~\ref{fig:system-visual}-D2). A gold line connecting the recalculated instance-level SHAP values (if a social group in a CBG is hovered) also appears beside the original purple line.
}

\cbgTable (Section~\ref{vis:cbg_view}): The corresponding row of the target CBG will become expandable, with sub-rows representing intervention strategies (Fig.~\ref{fig:system-visual}-B1).
Predicted changes to the segregation index and inflow proportions of social groups are visualized with thin gold bars overlaying the original bars. 
Users can save, edit, and delete strategies using the icons on the right side. 

\dorlingmap (Section~\ref{vis:map_view}): In glyphs, thinner gold flow arcs will overlay the original flow arcs to visualize flow changes resulting from interventions (Fig.~\ref{fig:system-visual}-C3).

==> archive/sections_for_pvis25_first_sub/06_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we present a quantitative analysis of our deep learning model. 
Then, we demonstrate two case studies developed with our experts.
We invited $E_B$, a marketing data scientist with three years of experience in income-based segmentation, to explore case 1 about income segregation.
We then invited our domain expert $E_A$, introduced in Section~\ref{prob_formulation}, to explore case 2 about partisan segregation.
Besides, we invited two more experts ($E_C$ and $E_D$) for the expert interviews detailed in Section~\ref{design_implication}.
$E_C$ has four years of experience in Geographical Information Systems (GIS), focusing on agent-based modeling (ABM) of segregation.
$E_D$ is a doctoral student who has been researching segregation on social media for two years.

\subsection{Quantitative Experiments}
\label{sec:model_evaluation}

% \parasum{Effectiveness of adaptation.}
% \subsubsection{Effectiveness of adaptation}
% To assess our adaptations to the original Deep Gravity model (social group segmentation and visitor characteristics inclusion as described in Section \ref{sec:model}), we ran a comparison experiment with five settings: 
% the original Gravity (G) and Deep Gravity (DG) models, DG adding social group segmentation (DG+S), DG including visitor characteristics (DG+V), and our adopted version which combines both adaptations (DG+S+V).
\parasum{Performance.}
\dyu{To assess our adaptations to the original Deep Gravity model (social group segmentation and visitor characteristics inclusion as described in Section \ref{sec:model}), we tested two baseline settings and three enhanced settings. 
The two baselines are the original Gravity (G) and Deep Gravity (DG) models. The three enhanced settings include DG with social group segmentation (DG+S), DG with visitor characteristics (DG+V), and the combination of both (DG+S+V), which is our final adopted version.}
Consistent with case 1, we used Houston data, segmented social groups by income, and included income and race as visitor characteristics.
\yy{
We assessed model performance using four metrics: Common Part of Commuters (CPC) measures the similarity between predicted and actual commuting patterns, while Jensen-Shannon Divergence (JSD) quantifies the difference between their distributions. Pearson Correlation indicates the strength of the linear relationship, and Root Mean Squared Error (RMSE) measures the average prediction error. 
Higher CPC and Pearson values, along with lower JSD and RMSE, indicate better model performance.
Table \ref{tab:algo-results} shows that DG+S+V achieved the best results across all metrics.
\footnote{We did a comprehensive evaluation of different cities and population densities. Please see the appendix for more information.}
}

% We then computed the Common Part of Commuters (CPC) using the following equation, consistent with the original work~\cite{simini2021deep}, to compare predicted flow $\hat{w}(v_i, v_j)$ with the actual $w(v_i, v_j)$.

\begin{table}[h!]

\centering
\vspace{-0.2cm}
\begin{tabular}{l|c|c|c|c}
\toprule
Model & CPC (↑) & JSD (↓) & Pearson (↑) & RMSE (↓) \\
\midrule
    DG+S+V & \textbf{0.6197} & \textbf{0.3497} & \textbf{0.7733} & \textbf{200.0248} \\
    DG+V & 0.6100 & 0.3580 & 0.6775 & 218.7619 \\
    DG+S & 0.6125 & 0.3565 & 0.7362 & 210.4794 \\
    DG & 0.5979 & 0.3684 & 0.6125 & 230.5540 \\
    G & 0.4605 & 0.4517 & 0.3862 & 245.4852 \\
\bottomrule
\end{tabular}
\vspace{-0.2 cm}
\caption{Performance comparison across different model settings}
\vspace{-0.5 cm}
\label{tab:algo-results}

\end{table}


\parasum{Time complexity.}
% \subsubsection{Time complexity}
We performed model training and inference on a 16GB MacBook Pro (Apple M1, no GPU). 
For Houston (around 1500 CBGs), in our case, individual model training took approximately 2 minutes. 
Therefore, we pre-trained models with expert-identified features offline. 
Model inference during what-if analysis (Section \ref{sec:model_what_if}) was fast (typically within 2 seconds), ensuring real-time feedback.

\begin{figure*} [t!]
 \centering 
 \vspace{-0.5cm}
 \includegraphics[width=\linewidth]{figs/case_v2.png}
 \vspace{-0.5cm}
 \caption{
     Case 2 - \systemname guided expert $E_A$ in analyzing partisan segregation and designing interventions. 
     He first compared the sociodemographics of communities (A1, A2) and searched for promising CBGs with intervention potential (B1, B2).
     He then analyzed the partisan preferences in mobility to the target CBG (C1, D1).
     He tried increasing food-related POIs (D2) to attract diverse visitors but it surprisingly worsened segregation (B4, C2).
     In contrast, increasing shopping facilities (D3) reduced segregation (B5).
     Finally, a combined intervention (D4) proved most effective (B6, C3).
 }
 \vspace{-0.6cm}
 \label{fig:system-case}
\end{figure*}

\definecolor{commAColor}{HTML}{51c44a} %6acc64
\definecolor{commBColor}{HTML}{4878d0}
\definecolor{commEColor}{HTML}{8c613c}
\newcommand{\commA}{Community \textcolor{commAColor}{\textbf{A}}\xspace}
\newcommand{\commB}{Community \textcolor{commBColor}{\textbf{B}}\xspace}
\newcommand{\commE}{Community \textcolor{commEColor}{\textbf{E}}\xspace}
% \newcommand{\commA}{Community \tcbox[on line, colframe=commAColor, colback=commAColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{A}\xspace}
% \newcommand{\commB}{Community \tcbox[on line, colframe=commBColor, colback=commBColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{B}\xspace}
% \newcommand{\commE}{Community \tcbox[on line, colframe=commEColor, colback=commEColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{E}\xspace}

\subsection{Case Studies}
Our cases focus on understanding and mitigating urban segregation in Houston City, the fourth-most populous city in the United States, known for its income inequalities~\cite{houstonincome} and partisan polarization~\cite{houstonpartisan}.

\subsubsection{Case1: A Prescription for Income Harmony}
We invited $E_B$, an experienced marketing data scientist working on income-based segmentation, to explore the first case about \textbf{income segregation}.
The income attribute uses the census data from 5-year American Community Survey and classifies the income into four groups from low to high: ``Under \$50K'', ``\$50K - \$100K'', ``\$100K - \$200K'', and ``Over \$200K''.
As suggested by $E_B$, the visitor characteristics in the input feature include both race and income.

\textbf{Overview of income disparities.} 
$E_B$ compared income signatures (\TIIpill) in the \commview (Fig. \ref{fig:system-visual}-A), and \commB (blue) emerged with a distinct segregation profile, characterized by a significant first box representing the low-income population (Fig. \ref{fig:system-visual}-A1-2).
In contrast, \commA (green), adjacent to Community B, exhibits greater economic diversity, with its signature showing a more even distribution across groups (Fig. \ref{fig:system-visual}-A1-1).
The \realmap (Fig. \ref{fig:system-visual}-C1) helped him localize them: \textit{``Community B is north of downtown, where neighborhoods face high poverty; Community A is located southwest of downtown, with booming areas like Sugar Land.''}

He then turned to the \flowmat (Fig. \ref{fig:system-visual}-A2) to understand inter-community connections (\TIpill), finding that Community B displays the most extreme income segregation in both incoming (last row) and outgoing (last column) mobility patterns.
Additionally, the lighter background shading of Community A's flow bar chart indicates minimal interaction with Community B.
\textit{``Despite their proximity, these communities rarely interact, deepening the segregation in activity spaces. How can we bridge this divide?''} $E_B$ wondered.
Therefore, he clicked Community B's label in the left column to focus on Community B.

\textbf{Targeting a CBG for intervention.}
Targeting specific CBGs within Community B for interventions (\TIIIpill), $E_B$ utilized the \cbgTable (Fig. \ref{fig:system-visual}-B), focusing on those with high segregation and bridging indexes.
Selecting the first CBG as the target triggered a series of visual updates: it was highlighted in black on both the \cbgTable and \realmap.
The \dorlingmap (Fig. \ref{fig:system-visual}-C2) and \featImpacts (Fig. \ref{fig:system-visual}-D2) also updated, displaying the target CBG's neighborhood connections and its feature impact.

\textbf{Analyzing inflow patterns and revealing intervention needs.}
$E_B$ further delved into inflow patterns to the target CBG, aiming to uncover the reasons behind its segregation (\TIVpill).
The \dorlingmap's \bubbleglyph (Fig. \ref{fig:system-visual}-C2) revealed a clear trend: the target CBG and nearby CBGs in Community B were dominated by the lowest income group (longest white arc). In contrast, five CBGs from Community A to the west had a more balanced income distribution but sent few visitors to the target CBG.

\yy{
The CPC bar showed the model predicted 70\% of the Common Part of Commuters to the target CBG accurately.
To investigate the disparity, the expert compared the \featImpacts (Fig. \ref{fig:system-visual}-D2) of the four social groups. 
To explore inter-group differences, he sorted the SHAP values by variance, revealing that health-related POI density ranked at the top.
The \featControl (Fig. \ref{fig:system-visual}-D1) showed no such amenities in the target CBG, while the \featImpacts revealed its stronger negative influences on the ``\$50K - \$100K'' and ``\$100K - \$200K'' groups.
This aligned with the expert's insight: \textit{``Health-related amenities tend to attract middle-class populations, as lower-income groups face affordability barriers and higher-income individuals often use private services. This market gap reinforces segregation.''}
}

\textbf{Testing an intervention strategy for integration.}
Inspired by his findings, $E_B$ turned to the \featControl (Fig. \ref{fig:system-visual}-D1) to design an intervention to reduce income segregation (\TVpill).
He simulated increasing health-related POIs in the target CBG by 1 unit per square kilometer.
The predicted outcome showed a 4.55\% decrease in segregation, as reflected in the expanded row of the \cbgTable.
Additionally, the \dorlingmap visualized an increased flow from Community A to the target CBG, depicted by longer gold arcs.
\yy{
Hovering over the arc for the ``\$100K - \$200K'' group in a neighboring CBG (Fig. \ref{fig:system-visual}-C3), $E_B$ observed a significant rise in the instance-level SHAP value for health POIs in the \featImpact (Fig. \ref{fig:system-visual}-D2), confirming that the intervention attracted more middle-class visitors.
}
\textit{``This highlights the importance of strategic placement,''} $E_B$ concluded, \textit{``Adding resources isn't enough – it's about targeting them to bridge communities. Much like expanding a product line to attract a wider customer base.''}

This case demonstrates how \systemname assists in understanding the urban segregation landscape, its possible causes, and how to design data-driven interventions. 
While tailored for social science, this example highlights the system's value for other fields, like marketing, where attracting diverse groups is a strategic goal.

\subsubsection{Case2: From Partisan Lines to Shared Spaces}
We invited $E_A$, our domain expert focusing on political polarization research, to explore the second case about \textbf{partisan segregation}.
For this analysis, we used the L2 Political Academic Voter File to obtain partisan membership data.
We classified non-Democratic or Republican parties as either ``Lean Democrat'' or ``Lean Republican,'' excluding independent or non-partisan individuals.
Proportions of these two partisan groups were then calculated for each CBG and included in the Sociodemographic Dataset (as described in Section \ref{sec:data_abstraction}). 
Following $E_A$'s suggestion, both income and partisan memberships were used as visitor characteristics in the input data to reveal the interplay between income levels and political beliefs.

\textbf{Searching for CBGs with intervention opportunities.}
After segmenting the city into communities (\TIpill), $E_A$ navigated through each community, searching for CBGs with intervention opportunities (\TIIpill{}, \TIIIpill). 
\commB (blue), predominantly Lean Democrat, initially caught his eye (Fig. \ref{fig:system-case}-A1). 
However, a closer look revealed a lack of CBGs with both a high segregation index and a high bridging index (Fig. \ref{fig:system-case}-B1), making it less ideal for his intervention plan.
Redirecting his focus, $E_A$ discovered \commE (brown), a politically mixed area (Fig. \ref{fig:system-case}-A2) with a promising landscape, with several CBGs flagged for both high segregation and bridging potential (Fig. \ref{fig:system-case}-B2). 
Therefore, he selected Community E and chose its first CBG for in-depth analysis.

\textbf{Analyzing partisan preferences in mobility.}
$E_A$ examined inflow patterns using the \dorlingmap (Fig. \ref{fig:system-case}-C1) and \featImpacts (Fig. \ref{fig:system-case}-D1) (\TIVpill), observing a clear Democratic majority in the target CBG. Republican-leaning neighboring CBGs, especially on the west side, showed minimal inflow, indicating a political divide. 
Sorting features by SHAP value variance, $E_A$ noted that the densities of shopping and food-related facilities had the most significant differential impact on mobility patterns for both groups. 
Despite the absence of both in the target CBG, $E_A$ inferred that Lean Democrats were more negatively affected by the lack of shopping venues, whereas Lean Republicans were more deterred by the absence of food outlets.
This observation aligns with the idea of ``political consumption,'' where consumer preferences reflect political identities: Democrats may favor niche shopping venues, while Republicans might prefer familiar food outlets.

\textbf{Exploring synergies to bridge divides.}
$E_A$ used the \featControl to test suitable interventions for segregation mitigation (\TVpill).
He began by increasing the shopping facility density to 3 units per square kilometer (Fig. \ref{fig:system-case}-D2), which resulted in a 6.44\% increase in the segregation index (Fig. \ref{fig:system-case}-B4).
Examining the \dorlingmap (Fig. \ref{fig:system-case}-C2), he observed,
\textit{``While we saw an increase in visitors from Republican-dominant CBGs, there was also a surge in visitors from the nearby Democrat-dominant CBGs, which worsened the segregation.''}

Resetting the current intervention, $E_A$ increased food facility density, noting a slight reduction in segregation. Advancing to 4 units per square kilometer (Fig. \ref{fig:system-case}-D3), he witnessed a 2.96\% drop (Fig. \ref{fig:system-case}-B5), with a notable increase in Republican-leaning visitors.
\textit{``Though both food and shopping facilities attract visitors, they have unique characteristics. 
Existing literature also shows different POIs have different contributions to segregation~\cite{zhang2023human}. Places that require more face-to-face interaction, in this case, the local grocery stores, can be more segregated.''} $E_A$ commented and recorded this intervention.

Intrigued by the interaction between shopping and food POIs, he simultaneously increased both types of amenities: shopping to 4 units per square kilometer and food to 3 units per square kilometer (Fig. \ref{fig:system-case}-D4).
Interestingly, this time, the segregation index did not increase because of the food facilities, but conversely, it decreased by 3.84\% (Fig. \ref{fig:system-case}-B6).
From the updated \dorlingmap (Fig. \ref{fig:system-case}-C3), it could be seen that Republican-dominated CBGs on the west side had more significant increases in visitor proportions to the target CBG.
\textit{``I thought the change would be linear and counteracted, but I didn't expect their combined effect to further decrease the segregation,''} $E_A$ pondered.
\textit{``Previously, we always treated POIs individually, and the combined effect of POIs is rarely touched, but such effect seems to be captured by the deep learning model. 
One hypothesis is those facilities co-create shared experiences of consumption and leisure, making the target CBG an even more inclusive multi-use community center for people holding different political beliefs.''}
Finally, $E_A$ thanked the system for shedding light on his future research: \textit{``In my following study, I may focus on this interesting effect of mixed-use area in the partisan segregation.''}

In summary, this case highlights that \systemname can help experts develop data-informed and feedback-driven urban planning insights to promote political integration and help researchers gain new insights that can be hard to reveal with traditional social science workflow.

==> archive/sections_for_pvis25_first_sub/07_discussion.tex <==
\section{Discussion}
The two case studies demonstrate the usability and effectiveness of \systemname in helping experts understand and mitigate different types of urban segregation.
To enrich our findings further, we interviewed two more experts ($E_C$ and $E_D$).
We presented the case study results and invited them to explore the system freely, collecting their feedback.
% $E_C$ specializes in Geographical Information Systems (GIS) with a focus on agent-based modeling (ABM) of human mobility.
% Meanwhile, $E_D$ is a doctoral student in social science, focusing on online segregation.

\subsection{Design Implications}
\label{design_implication}
We summarize insights from the feedback of four experts.

\textbf{Applications and target users.} 
All experts praised the usefulness of \systemname, suggesting its potential applications beyond the current user base.
For the \commpill unity and \cbgpill-level analysis, $E_B$ and $E_C$ highlighted the progressive workflow as an efficient tool that enables geospatial analysts to rapidly explore the complex mobility data within unfamiliar cities without extensive custom coding.
$E_D$ expected to utilize the \commview and \dorlingmap to visualize communities and echo chambers on online social media.

For the \poipill-level Analysis, $E_A$ and $E_B$ saw it as a bridge between researchers and decision-makers, offering benefits in various scenarios. 
% $E_A$ shared a compelling example of using its simulation power to inform urban decision-making: 
% \textit{``If I could use this system to simulate the impact of a community center demolition and present it to the municipal office, the decision-making process might have been entirely different.''}
Besides social scientists, $E_A$ shared that social activists and NGOs who want to promote social well-being in communities could use the system to assess the potential impact of municipal policies: \textit{``Imagine using \systemname before the decision of demolishing a community center and sharing these simulations with the municipal office; it might influence discussions and final planning.''}
$E_B$ underscored the system's value for professionals in fields like marketing.
He shared that he previously used TensorFlow's What-If tool but found its output limited and difficult to contextualize for clients. However, \systemname offers visually appealing results and intuitive comparisons, greatly enhancing presentations.

\textbf{Transparency and trust in what-if analysis.}
$E_C$, specializing in spatial agent-based modeling (ABM), praised the deep-learning model's ability to capture complex human behavior (in case 2).  However, he highlighted a key difference between deep learning and ABM: the issue of transparency. \textit{``ABM, while potentially oversimplifying human behavior, grants experts direct access to agent attributes and states~\cite{liu2022abm}, allowing for greater transparency and control over experiments.''}  
Therefore, for future projects targeting experts who value rigorous experimental control,  we suggest carefully balancing the benefits of deep learning models with the explainability of ABM.
One potential hybrid approach is integrating ABM into mobility data modeling, leveraging the complex behavior captured by deep learning~\cite{turgut2023framework}.

Regarding the trustworthiness of what-if analysis, $E_D$ expressed concerns about the lack of longitudinal validations.
While long-term evaluation is ideal for planning, gathering such data in a controlled environment is impractical for dynamic urban settings.
To address this, our system employs feature impact analysis and CPC scores to help experts assess the reliability of predictions.
All experts agreed that these tools improved their confidence by providing insights into the model’s reasoning, aligning with their domain knowledge.
$E_A$ mentioned that a CPC above 60\% was typically sufficient to proceed, as this indicates the model captures meaningful correlations between environmental features and movement patterns.
Although long-term validation remains a challenge, $E_B$ emphasized that even short-term insights, such as those provided by TensorFlow's What-If Tool, can still guide practical interventions when combined with expert knowledge.

\textbf{Feasibility consideration in ``technology for social good.''}
Both $E_B$ and $E_C$ appreciated our careful consideration of the feasibility of urban planning interventions during the design phase. 
The focus on identifying areas with high potential (using TOPSIS ranking) and implementing targeted interventions was seen as a key strength for promoting a greater chance of real-world impact. 
This approach, prioritizing practical implementation, can be borrowed for other technology-for-social-good projects, helping to narrow down targets and increase feasibility.

\subsection{Limitations and Future Works}
We introduce the limitations of our system and future work.

\textbf{Lack of temporal dimension.}
Currently, \systemname operates on a static snapshot of urban mobility and segregation patterns, not accounting for temporal variations. 
Urban dynamics, like seasonal changes, can significantly impact segregation patterns. 
In the future, we will extend our deep learning model to analyze time-series mobility data and incorporate visualization techniques such as the Spatio-Temporal Graphs~\cite{von2015mobilitygraphs} to capture the temporal dynamics of segregation patterns.

\textbf{Possible bias in the demographic composition of visitors.}
We currently infer visitors' sociodemographic characteristics based on residents' census data. While this is a common practice in social science~\cite{zhang2023human, athey2021estimating}, it can introduce bias.
% For example, wealthy people living in an economically diverse CBG might primarily visit wealthy areas. However, under our current method, we'd estimate they also visit places frequented by other residents of the CBG, potentially underestimating income segregation.
In the future, we aim to improve data accuracy by obtaining individual-level mobility data (\eg, telecommunication data~\cite{wu2015telcovis}) and integrating more fine-grained imputation methods, such as using housing prices~\cite{nilforoshan2023human} to infer sociodemographics.

\textbf{Coarse-grained POI categories.}
The current 12 broad POI categories limit the granularity of insights provided for policymaking.
$E_A$ and $E_B$ suggested the value of modeling fine-grained categories within the current main categories. For example, distinguishing between fast food and fine dining restaurants might reveal significant differences in their impact on mobility~\cite{garcia2024effect}. 
However, this presents a challenge due to the large number of fine-grained POI categories (approximately 200 in our current SafeGraph dataset).
In the future, we plan to work closely with social scientists to develop a refined POI taxonomy. This taxonomy will balance comprehensiveness with a focus on the subcategories most impactful to segregation, enabling more accurate modeling.

\textbf{More contextual geographical information.}
$E_C$ highlighted the need for additional geographic layers to inform the feasibility of urban planning interventions.
This includes elements like transportation networks and natural resources.
In the future, we will develop a more advanced \mapview showing multi-layered GIS data to provide a richer context for more accurate decision-making during \poipill-level analysis.

==> archive/sections_for_pvis25_first_sub/08_conclusion.tex <==
\section{Conclusion}
In this work, we introduce \systemname, a visual analytics system that leverages human mobility data to empower in-depth exploration and mitigation of urban segregation.
Our system combines a data analysis pipeline with an interactive interface featuring novel visualizations to support a three-level analysis workflow, enabling experts to examine segregation patterns from overview to detail and iteratively design feedback-driven urban planning interventions.
A quantitative evaluation demonstrates our model's accuracy in modeling mobility data and its capabilities for real-time interactive analysis.
Case studies and expert interviews further highlight \systemname's value in helping social scientists and policymakers uncover complex segregation patterns and design inclusive, equitable urban spaces.

==> archive/sections_for_vis24__old_/00_abstract.tex <==
% dyu
\abstract{
Urban segregation is an increasingly critical social problem, creating invisible barriers that exacerbate social inequalities within cities. Existing segregation studies, which predominantly focus on residential areas, fail to fully capture the complex dynamics of segregation across various ``activity spaces'' such as work, leisure, and social interactions.
The proliferation of GPS-based human mobility data offers a fresh perspective for a detailed analysis of segregation within a broader area, but it also introduces challenges to existing statistical approaches in understanding the complex dynamics and local nuances of urban segregation. 
This work introduces \systemname, a novel visual analytics system that enables comprehensive and multi-level analyses of urban segregation and the development of targeted, data-driven interventions. 
In particular, we develop a deep learning model to predict mobility patterns across different social groups based on environmental features while applying explainable AI techniques to reveal the impacts of these features on segregation levels. 
\systemname integrates a set of innovative visualizations that empower users to explore segregation patterns from broad overviews to fine-grained detail, and then to design and evaluate urban planning interventions with real-time feedback. 
We conduct a quantitative evaluation to demonstrate the accuracy and time complexity of our algorithm. 
Two case studies and expert interviews with social scientists and urban analysts are further conducted to validate \systemname's efficacy, confirming its potential to significantly inform and guide urban planning efforts toward creating more inclusive and equitable urban environments.
}

% V2.0
% \abstract{
% Segregation is a critical social problem, isolating a city into filter bubbles that limit opportunities and hinder social equality. 
% While traditional approaches analyze residential segregation, the emergence of large-scale human mobility data allows more fine-grained segregation study within ``activity spaces'' (\eg, work, leisure, and social areas).
% However, existing social science methods fall short in this data with a focus on global statistics, lacking detailed insights for holistic understanding and simulation for informed policy-making.
% This work introduces \systemname, an interactive visual analytics system that empowers social scientists and policymakers to conduct multi-level segregation analyses and develop data-driven interventions to mitigate segregation. 
% \systemname leverages a deep learning model to predict mobility patterns across social groups based on environmental features, while explainable AI techniques reveal feature impacts on segregation levels.
% In addition, a suite of coordinated visualization views is proposed to aid exploration. 
% Experts can explore how environmental features shape local spatial interactions and dynamically adjust features to receive real-time feedback on the interface, facilitating an iterative process to refine data-driven interventions.
% We conduct a quantitative evaluation to show the accuracy of our algorithm.
% Two case studies and expert interviews with social scientists and urban analysts are further conducted to validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive environments.
% }

% V1.0
% \abstract{
% Segregation is a critical social problem, isolating a city into different filter bubbles that hamper community integration and limit opportunities for underprivileged groups. 
% This makes understanding and mitigating segregation a vital goal for social scientists and policymakers to foster social equality.
% Recently, the emergence of large-scale human mobility data has provided new opportunities to study fine-grained segregation within ``activity spaces'' — areas where people work, socialize, and leisure beyond traditional residential locations.
% However, despite this data availability, existing approaches remain limited by their focus on global statistics, lacking detailed insights for holistic understanding and effective simulation for feedback-driven policy-making.
% Hence, in this study, we address this gap by introducing \systemname, an interactive visual analytics system that empowers social scientists and policymakers to conduct nuanced analyses of urban segregation and to develop effective interventions through simulation-driven insights. 
% \systemname features a three-level progressive analysis workflow: starting with a segregation overview, delving into the detailed factors that drive it in Census Block Groups (CBGs) with intervention potential, and ending with formulating and evaluating interventions to mitigate segregation.
% In addition, a series of coordinated visualization views are proposed to assist users throughout the analysis workflow: a Community View with community signatures for demographic comparison, a CBG View for in-depth analysis of CBGs, integrated with a metaphor-based Map View for understanding neighborhood interactions, and a What-If View for evaluating intervention strategies.
% Through case studies and expert interviews, we validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive and equitable environments.
% }

%% Abstract section.
% V0
% \abstract{%
% Segregation is a severe social problem today that hampers community integration and diversity, isolating a city into different filter bubbles. This makes understanding and mitigating segregation a vital goal for social science researchers and policymakers.
% Recently, the availability of large-scale human mobility data has provided new opportunities to measure more fine-grained segregation in activity space.
% However, there lacks an efficient visual analytics approach for in-depth analysis of segregation and formulation of feedback-driven intervention strategies. 
% In this study, we address this gap by introducing \systemname, an interactive visual analytics system designed to empower social scientists to understand mobility-based urban segregation and develop effective urban planning interventions. 
% \systemname features a comprehensive three-level analysis workflow, allowing for an initial exploration of overall segregation, followed by an in-depth examination of the factors driving it, and concluding with the formulation and assessment of intervention strategies.
% In addition, a series of coordinated visualizations are proposed, including a Community View with unique community signatures for efficient demographic comparison, a CBG View coupled with metaphor-based Map View to reveal environmental influences on the segregation in a specific CBG and its interactions between neighboring areas, and a What-If View to enable interactive exploration and assessment of various intervention strategies.
% Through case studies and expert interviews, we validate \systemname's efficacy, showcasing its potential to guide urban planning toward more inclusive and equitable environments.
% }

==> archive/sections_for_vis24__old_/01_introduction.tex <==
\section{Introduction}

Imagine invisible lines, not physical walls, dividing a city; residents are segregated based on their wealth, race, and political beliefs. People live in bubbles and rarely interact with those who do not share similar sociodemographic backgrounds. Such division is known as \textbf{urban segregation}~\cite{white1986segregation}, not by a geographical split, and reinforces social inequalities. 
% It acts as a barrier to resources and opportunities for those from vulnerable groups and hinders the collective inclusivity and vibrancy of our societies. 
To reshape cities into more inclusive and equitable spaces, social scientists and policymakers have devoted their efforts to understanding these invisible barriers and proposing effective urban planning interventions to mitigate and dismantle them~\cite{chetty2020income, nilforoshan2023human}.

The study of urban segregation analysis in social science primarily relied on the census statistics (e.g., racial composition) of the residential areas~\cite{white1986segregation} to understand the segregation situation in a city. 
This traditional approach, while informative, provides a relatively narrow lens that only focuses on residential environments. 
It overlooks the full picture of human interaction beyond residential areas, such as workplaces and social venues, potentially biasing the analysis. 
The recent availability of GPS-based human mobility data is broadening segregation studies from ``residential space'' to ``activity space''~\cite{cagney2020urban},  offering a more comprehensive view of how people experience segregation in their daily routine~\cite{wong2011measuring, browning2017socioeconomic, zhang2023human}. 
% Such oversight can lead to possible bias in the analysis, potentially missing its full impact.
% With the recent availability of GPS-based human mobility data, segregation studies are shifting the focus from solely ``residential space'' to ``activity space''~\cite{cagney2020urban}. The mobility data allow a more comprehensive view of how people experience segregation in their daily routine~\cite{wong2011measuring, browning2017socioeconomic, zhang2023human}. 
% including activities such as working, socializing, and shopping~\cite{wong2011measuring, browning2017socioeconomic, zhang2023human}. 
For example, researchers try to explain the motivations behind mobility segregation by indexing the segregation and modeling the human daily activity trajectories~\cite{moro2021mobility} and suggest urban planning interventions to bridge diverse communities~\cite{nilforoshan2023human}.

Despite global segregation statistics offering broader insights, they fall short of capturing the intricate local dynamics of segregation and the complex interactions between different spatial units. The absence of both a \textit{data-informed} and \textit{feedback-driven} approach makes it difficult for social scientists and policymakers to precisely evaluate and fine-tune intervention strategies. 
% thus hindering their ability to effectively counter the multifaceted nature of urban segregation.
Visual analytics (VA) emerges as a crucial approach to overcome the aforementioned limitations through intuitive visual representations in different levels of detail and interactive interfaces that support trial and error. Nevertheless, designing an effective VA system to bridge the current research gap is non-trivial. First, a city's mobility dataset typically comprises thousands of spatial units with potential flows between any two.
Despite aggregation techniques helping grasp overall mobility networks~\cite{von2015mobilitygraphs, zhou2018visual, liu2019tpflow}, obtaining detailed insights for precise urban planning through suitable visualizations and computational support is still a significant challenge.
% Although aggregation techniques aid in understanding overall-level mobility networks~\cite{von2015mobilitygraphs, zhou2018visual, liu2019tpflow}, achieving granular insights through appropriate visualization designs and computational supports for precise urban planning interventions remains a formidable challenge.
Some VA systems have shown promise in urban planning contexts, such as optimizing location choices~\cite{liu2016smartadp, chen2023fslens} or enhancing bus network efficiency~\cite{weng2020towards}. However, they are not equipped for urban segregation analysis, which requires navigating the intricate socio-spatial fabrics that define cities. 
Second, unraveling the complex correlations between environmental features and mobility patterns
demands a nuanced approach due to the multifaceted, nonlinear, and spatially diverse nature of these correlations~\cite{athey2021estimating}. 
Existing visualizations can display the impact of geographical context on a dependent variable within single regions~\cite{lei2023geoexplainer, yu2023neighviz}, but they fail to address mobility flows between regions.

To address the challenges outlined, we propose \systemname, a visual analytics system tailored to understand and mitigate urban segregation through the lens of mobility data.
Over a year-long collaborative effort with a computational social scientist, the system is designed to meet the complex demands of urban segregation analysis effectively. 
In particular, we develop a deep learning model based on Deep Gravity~\cite{simini2021deep} to predict mobility flows using environmental features. 
To explain the influence of various features on mobility among different social groups, we integrate Partial Dependence Plots (PDP)~\cite{friedman2001greedy, hastie2009elements} into our model. 
These plots isolate and display the impact of distinct features on mobility trends.
Additionally, we introduce a radial-layout visualization, combining PDP results with real environmental data to show how urban elements affect mobility in specific areas. 
Leveraging our deep learning model, \systemname further offers a dynamic what-if functionality, enabling users to interactively adjust parameters and explore the effects of various urban planning choices, such as the addition or modification of community facilities.

In summary, the main contributions of this work are as follows:
\begin{itemize}[itemsep=0.05pt, leftmargin=*]
% \begin{itemize}[noitemsep, leftmargin=*]
    \item
    We systematically delineate the problem domain for understanding and mitigating urban segregation using mobility data and present three levels of socio-spatial analysis.
    
    \item 
    We introduce a comprehensive data analysis pipeline that allows for mobility-based community detection, segregation calculation, mobility flow prediction, and feature influence explanations. The pipeline also supports what-if analyses, laying the groundwork for guiding precise urban planning interventions.
    
    \item 
    We develop \systemname, a visual analytics system with novel visualization designs, such as metaphor-based bubble glyphs, enabling interactive exploratory analysis of segregation patterns and the testing and evaluation of potential urban planning interventions.

    \item 
    % \dyu{Evaluation: case studies} 
    We evaluate \systemname with two case studies and interviews with domain experts to show the system's effectiveness and usability. 
\end{itemize}


==> archive/sections_for_vis24__old_/02_related_works.tex <==
\section{Related Works}

\subsection{Segregation Analysis in Mobility Data}
\label{sec:related_segregation}
% Understanding the segregation pattern in human mobility is crucial for designing inclusive cities that promote equitable access to resources and opportunities. 
Two approaches are typically applied by social scientists to analyze segregation in mobility data: (1) the index-based approach, which measures the segregation level, and (2) the model-based approach, which uncovers underlying reasons for the segregation. 
% To analyze the segregation in mobility data, social scientists typically adopt a \textbf{segregation index} to describe the segregation situation and develop a \textbf{mobility model} to uncover underlying reasons for the segregation.

\textbf{Segregation index} 
is a straightforward approach as an indicator to understand the segregation level in human mobility data.
The index is usually computed based on the demographics of the group of people who visit a place during a period of time. 
The computation formula of the segregation index is diverse, which can be information entropy~\cite{huang2022unfolding}, isolation index~\cite{white1986segregation, athey2021estimating}, or just distribution unevenness~\cite{zhang2023human, moro2021mobility}. 
Depending on the research topic, the main subject of the segregation can involve different attributes, including income, partisan~\cite{zhang2023human}, race~\cite{athey2021estimating}, or a combination of them~\cite{huang2022unfolding}.
% For example, to study the partisan segregation in human mobility, Zhang \et~\cite{zhang2023human} develop two indices to measure each place's partisan segregation brought by its visitors and partisan segregation experienced by its residents based on the unevenness of the partisan distribution in an area. Their study indicates that some communities with certain characteristics (\eg, black, liberal, low-income, non-immigrant, more public transit-dependent, and central city) are experiencing partisan segregation.
However, the segregation index, being merely an aggregated descriptive metric, does not explain the underlying reasons for the segregation patterns in mobility data.

\textbf{Mobility models} offer researchers a detailed examination of the features influencing mobility and segregation patterns.
A classic model is Exploration and Preferential Return (EPR)~\cite{song2010modelling}, which uses two key parameters, exploration (visiting new places) and preferential return (revisiting previously visited locations), to model the dynamics of human movement trajectories.
Moro \et~\cite{moro2021mobility} extend the EPR by adding a parameter that quantifies an individual motivation to visit new places where their income group is in the minority. 
% The estimated model parameters reveal a strong association between people's experienced income segregation and their tendency towards exploring places where they are in the socioeconomic minority.
Nevertheless, modeling complex human behaviors with few parameters may oversimplify the complexity of mobility patterns and their driving factors.
In contrast, a more generic model, Deep Gravity~\cite{simini2021deep}, employs a comprehensive set of features (\eg, the density of different facilities and demographic information) and uses a deep neural network to predict mobility flow probabilities between places. 
% It leverages Explainable AI techniques, such as SHAP values, to reveal the influence of each environmental feature on mobility predictions.
% While DeepGravity initially does not include demographic or segregation features, its adaptable architecture allows for integrating such factors.
Yet, the complexity of neural networks trained on extensive datasets complicates understanding segregation patterns' key features and developing solutions to mitigate segregation.

In this work, we propose a data analysis pipeline that computes the segregation index and models the impact of environmental features on mobility flows using an adapted Deep Gravity model. 
We also develop a VA system with tailored interaction and visualization designs to support what-if analysis, seamlessly integrating with the data analysis pipeline.


\subsection{Human Mobility Visualization}
Human mobility analysis has been widely studied in the visualization community~\cite{deng2023survey}. 
Here, we mainly discuss the most relevant literature about mobility data visualization and mobility model visualization.

\textbf{Mobility data visualization} often uses origin-destination (OD) flow map~\cite{guo2014origin} to visualize an individual’s movement trajectories.
However, OD flow maps can become visually cluttered with dense data. To address this, researchers have developed alternative visualization techniques such as matrix representations, where each cell indicates flow volume while preserving spatial layout~\cite{wood2010visualisation, yang2016many}. 
Additionally, techniques leveraging data mining, including clustering~\cite{von2015mobilitygraphs, liu2019tpflow, shi2020urbanmotion} and Word2Vec~\cite{zhou2018visual}, have been employed to aggregate mobility data and distill key insights, thereby enhancing visualization clarity and interpretability.
Other mobility visualization work further incorporates semantic information, such as point of interest (POI) information~\cite{zeng2017visualizing} and social media text~\cite{chen2015interactive, krueger2019bird}, enriching the contextual understanding of mobility patterns.
However, a notable gap in the literature is the insufficient integration of demographic data into mobility visualization, which is essential for understanding underlying social dynamics such as income and racial inequality~\cite{athey2021estimating, moro2021mobility} and partisan polarization~\cite{zhang2023human}.

\textbf{Mobility model visualization}, primarily studied in the transportation domain, can facilitate understanding the driving factors of mobility patterns.
For instance, visualizing congestion predictions generated by deep learning models can assist experts in analyzing and predicting congestion scenarios~\cite{lee2019visual} and even refining the models~\cite{jin2022visual}.
Meanwhile, TCEVis~\cite{dong2023tcevis} employs SHAP values to offer explainable insights into the features influencing traffic congestion.
However, these approaches generally model the mobility behavior of the entire population, overlooking social group distinctions.

Our work not only visualizes the mobility patterns of diverse social groups but also incorporates these distinctions into mobility modeling. 
This approach allows for a visual comparison of the factors driving segregation among different social groups, enhancing the understanding of mobility dynamics within a sociodemographic context.

\subsection{What-If Analysis}
What-if analysis empowers users to explore the predictive models by adjusting input features, thereby understanding the model's behavior under various hypothetical scenarios.
Visual analytics systems enhance this exploration by facilitating interactive feature adjustments to observe their impact on predictions~\cite{krause2016interacting, wexler2019if, cheng2021vbridge}.
In the urban planning scenario, what-if analysis is widely embedded in many planning support systems, such as $\rm{What-If?}^{TM}$~\cite{klosterman2008whatif} and CommunityViz~\cite{janes2008communityviz}, as well as traffic analysis systems~\cite{andrienko2016leveraging} and public policy simulators~\cite{yang2022epimob, usman2022multiscale}. 
These systems facilitate data-driven decision-making by enabling stakeholders to simulate and evaluate the consequences of various urban design scenarios. 
However, a common limitation among these tools is their lack of focus on the goal of integrating diverse social groups through urban planning interventions.
CityScope~\cite{alonso2018cityscope} more closely aligns with our objectives by offering a tangible interface that promotes urban performance metrics, including the exposure diversity of social groups.
Nevertheless, the agent-based modeling behind CityScope, relying on parameters distilled from surveys or regression~\cite{grignard2018impact}, may oversimplify the diverse social and environmental nuances of urban settings.

In our work, we develop a deep learning model to capture complex correlations between environmental features and segregation, enabling our what-if analysis to provide real-time feedback on the effectiveness of user-defined interventions. We further presented a set of tailored visualizations based on superposition approaches to support comparative analysis between different intervention strategies.

==> archive/sections_for_vis24__old_/03_background.tex <==
\section{Background}

% In this section, we first introduce the analytical goals distilled together with the expert, which derive five visualization design tasks. We then introduce the system overview.

\subsection{Problem Formulation}
\label{prob_formulation}

Over the past year, during our system design phase, we closely collaborated with social scientist $E_A$ to shape the design of \systemname.
$E_A$ is an experienced researcher in using human mobility data for urban segregation analysis with a number of relevant publications focusing on the causes and mitigation of partisan segregation. 
During our system's evaluation phase, we also involved experts $E_B$, $E_C$, $E_D$ (detailed in Section~\ref{sec:evaluation}).
Through monthly discussions with $E_A$ and extensive literature reviews, we found that traditional urban segregation studies mainly focus on computing segregation indices and using regression analyses to associate environmental features with segregation levels~\cite{zhang2023human, huang2022unfolding, athey2021estimating}.

These methods offer an overview of segregation patterns, but examining detailed local mobility dynamics and the interactions between spatial units often requires labor-intensive, ad-hoc coding and analysis, which can be time-consuming.
To address these limitations, we have first identified two primary analysis goals, \textit{Community-level Analysis} and \textit{Census Block Group (CBG)-level Analysis}, to facilitate a comprehensive exploration and analysis of segregation patterns from an overview to detailed dynamics in mobility data.
In our study, a CBG is a basic spatial unit like a small, precisely defined neighborhood with 600-3000 residents, while a community refers to a group of CBGs like a larger district within a city, where people tend to interact more frequently within those areas.


During our discussions, $E_A$ expressed keen interest in identifying strategic urban planning methods to counteract the observed segregation, alongside a straightforward approach to assess the impact of proposed plans.
Even though there are existing tools for simulating the effects of urban policies~\cite{klosterman2008whatif, janes2008communityviz, alonso2018cityscope}, he commented they are not seamlessly integrated with segregation analysis for data-driven decision-making.
Also, among various urban planning interventions, $E_A$ suggested adjusting different types of Points of Interest (POIs) as a practical strategy for addressing segregation.
Consequently, we identified the third goal: \textit{Point of Interest (POI)-level Analysis}, to allow for interactive exploration and assessment of POI modifications to promote inclusivity.
Overall, we have summarized three analysis goals below.

\textbf{\commpill unity-level Analysis} The expert aims to obtain an overview of the city's segregation dynamics at a community level, identifying a focus area for deeper analysis. 
This involves examining the mobility patterns and sociodemographic characteristics of communities.

\textbf{\cbgpill-level Analysis} Within the focus community, the expert wants to pinpoint candidate CBGs to mitigate segregation. 
Therefore, the expert hopes to efficiently identify these CBGs that present opportunities for intervention and explore how their features influence visitor flows from different social groups.

\textbf{\poipill-level Analysis} The expert aims to strategically adjust POIs in a target CBG to mitigate segregation and promote inclusivity.
The expert wants to explore and compare the effectiveness of different POI adjustments in promoting inclusivity.

\subsection{Design Requirements}
\label{sec:03_Background_VisualizationDesignTasks} 

We have further identified five system design requirements with $E_A$, in order to support the above three-level socio-spatial analysis goals: 
% In light of the goals above, we have then collaborated with $E_A$ through iterative interviews, and subsequently, we derived five visual analysis tasks to support the three-level socio-spatial analysis above:

\hangpara{2em}{1}
\TIpill{} \textbf{Segment and characterize communities.} 
The system should facilitate the identification of mobility-based communities. 
It should further characterize these communities using various statistics of the flows between them to help the expert understand how they are interconnected. 

\hangpara{2em}{1}
\TIIpill{} \textbf{Compare sociodemographics across communities.} 
The system should support the comparison of sociodemographic attributes among communities, including both their residents and visitors, to help the expert identify a community exhibiting significant segregation in activity space for further investigation.

\hangpara{2em}{1}
\TIIIpill{} \textbf{Identify CBGs with intervention potential.} 
Within the selected community, the system should list the CBGs ranked by multiple segregation-related criteria.
This will assist the expert in pinpointing CBGs that show significant segregation levels and have a high potential for effective interventions. 

\hangpara{2em}{1}
\TIVpill{} \textbf{Analyze target CBG inflow \& influential features.} 
After a target CBG from the candidate list is selected, the system should provide a detailed analysis of its inflow patterns of different social groups, highlighting how key environmental features influence these patterns and contribute to segregation.

\hangpara{2em}{1}
\TVpill{} \textbf{Simulate urban planning interventions.} 
The system should support the expert to experiment with ``what-if'' scenarios by modifying POI features in the target CBG.
It should then simulate and visualize the real-time impact of these changes on mobility patterns and segregation levels, facilitating the expert's assessment of interventions for inclusivity.

\begin{figure} []
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/system overview.png}
 \vspace{-0.5cm}
 \caption{
    System overview - \systemname comprises three modules: Data, Analysis Pipeline, and Visualization, to support interactive segregation analysis (\commpill{} and \cbgpill) and iterative intervention development (\poipill).
 } 
 \vspace{-0.4cm}
 \label{fig:system-overview}
\end{figure}

\subsection{System Overview}
\label{sec:system-overview} 
To address the identified requirements, we developed \systemname, an open-source human-in-the-loop VA system\footnote{\url{https://anonymous.4open.science/r/inclusiviz/}} consisting of three modules: the Data module, the Analysis Pipeline module, and the Visualization module as shown in Fig.~\ref{fig:system-overview}.
The Data module stores data in a database in the structures as detailed in Section \ref{sec:data_abstraction}.
The Analysis Pipeline module integrates mobility-based community detection (Section \ref{sec:community_detection}), segregation measures (Section \ref{sec:segregation_measures}), and a deep learning model (Section \ref{sec:model}) enhanced with explainable AI techniques that pinpoint influential features (Section \ref{sec:model_pdp}) and evaluate the impact of user-defined urban planning interventions (Section \ref{sec:model_what_if}).
Finally, the Visualization module consists of four coordinated views (Section \ref{sec:05_visual_design}) enabling users to explore analysis results, experiment with hypothetical interventions, and receive real-time feedback on potential outcomes.



==> archive/sections_for_vis24__old_/04_data_analysis.tex <==
\section{Data Analysis Pipeline}
\label{sec:04_Data_Analysis}
In this section, we first introduce the data abstraction in our study, and we elaborate on the components in our analysis pipeline that analyze segregation patterns and model the mobility data.

\subsection{Data Abstraction}
\label{sec:data_abstraction}
We mainly used three types of datasets gathered from a single city.
We primarily focus on the Census Block Group (CBG) as our core spatial unit, a detailed division commonly used in social science research, typically encompassing 600 to 3000 residents according to the U.S. census. 
This choice of unit ensures fine-grained analysis, but our system is adaptable to other spatial divisions, such as England's Lower Layer Super Output Areas (LSOA). 
Below is a description of each dataset:

\begin{itemize}[itemsep=0.05pt, leftmargin=*]
    \item \textit{Mobility Dataset} contains the aggregated movement of individuals between various CBGs over one year. 
    It is structured as a directed weighted graph $ G = (V, E) $, where each node $ v \in V $ is a CBG, and each edge $ (v_i, v_j) \in E $ represents the flow of individuals from CBG $ v_i $ to $ v_j $, weighted by the count of these individuals, $ w(v_i, v_j) $.
    In our study, we utilized data provided by $E_A$, aggregated from SafeGraph. 
    This dataset encompasses large-scale monthly mobility flows from origin CBGs to destination places, collected from anonymous mobile devices, covering approximately 10\% of the entire U.S. population.
    
    \item \textit{Sociodemographic Dataset} contains population characteristics of each CBG (\eg, income and race)
    For an attribute $ D $ (\eg, income level), it has a matrix $ S_D = [s_{id}] $, where $ s_{id} $ is the population count of a social group $ d \in D $ (\eg, \$ 50K-100K income group) of CBG $i$.
    We obtained the data from the 5-year American Community Survey and L2 Political Academic Voter File.
    
    \item \textit{POI Dataset} contains the density (number per square kilometer) of each type of POI in each CBG. 
    It is formatted as a matrix $ P = [p_{ip}] $, where $ p_{ip} $ represents the density of POI type $ p $ in CBG $ i $.
    In our study, this dataset is also sourced from SafeGraph, containing 12 major POI types such as food, shopping, work, health, and others.
\end{itemize}

\begin{figure}
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/data_v0.png}
 \vspace{-0.5cm}
 \caption{
    In the data analysis pipeline, the Segregation Measures (A) computes each CBG's Segregation Index (1) and Bridging Index (2), and then ranks them using Dual-Attribute Ranking (3).
    The Mobility Data Modeling (B) trains a Deep Learning Model for a social group (1), enhanced with Partial Dependence (2) and What-If Analysis (3) modules.
    % (A) The computation of two segregation measures: 1. segregation index and 2. bridging index.
    % (B) Mobility Data Modeling, consisting of 1. a Deep Gravity Model for each social group, 2. a Partial Dependence Plots module, and 3. a What-If Analysis module.
 }
 \vspace{-0.4cm}
 \label{fig:data_analysis}
\end{figure}

\subsection{Mobility-based Community Detection}
\label{sec:community_detection}

In segregation studies, clustering spatial units in a city into communities with high internal movement but limited external interactions can effectively reveal data-driven social boundaries, offering a clear overview of segregated areas~\cite{huang2022unfolding, burdick2020socially}.

For community detection in directed weighted graphs that align with our \textit{Mobility Dataset}, multiple community detection algorithms are available, including flow-based InfoMap~\cite{rosvall2009map} and modularity-based Leiden~\cite{traag2019louvain}.
These algorithms offer distinct advantages: the Leiden algorithm tends to segment larger community structures, while the InfoMap algorithm tends to identify sub-communities~\cite{gibbs2021detecting}. 
Considering our objective of maintaining a manageable number of communities for an interpretable overview as the initial analysis, we adopt the Leiden algorithm.
The algorithm takes an edge list, where each entry contains the source CBG $v_i$, the destination CBG $v_j$, and the flow weight $w(v_i, v_j)$, as input and iteratively optimizes modularity by reassigning CBGs to communities.
% The Leiden algorithm initially assigns every CBG as an independent community. Then, the algorithm iteratively moves CBGs between communities to enhance the overall modularity.
% After achieving local optimality, it combines CBGs in communities and rebuilds the network, and repeats. The algorithm concludes when there's no further improvement in modularity.
To focus on significant mobility patterns, we apply a customizable flow threshold $w_{min}$ to retain only edges where $w(v_i, v_j) \geq w_{min}$.
For interpretability, we focus on the 10 largest communities, grouping the remaining CBGs into an ``others'' category.


\subsection{Segregation Measures}
\label{sec:segregation_measures}

\subsubsection{Segregation Index}
The segregation index (Fig.~\ref{fig:data_analysis}-A-1) is a common practice to quantify the segregation level of visitors in an area.
% A more uniform distribution indicates a more inclusive area with a lower level of segregation in the activity space, implying that individuals visiting this area interact with a diverse range of people.
Different formulas have been developed to calculate the segregation index using mobility data as discussed in Section \ref{sec:related_segregation}.
In this study, we adopt the distribution unevenness recommended by our expert due to its ease of interpretation~\cite{zhang2023human}.

For any target CBG $v_{target}$ visited by $N$ source CBGs, to calculate its segregation index of a sociodemographic attribute $D$, we first determine the proportion of residents in each social group $d$ in each source CBG $v_i$ as $\theta_{id}$. 
Next, for each social group $d$, we calculate the proportion of visitors from $d$, $\pi_d$, using the equation:

\begin{equation}
\label{equation:segregation_prop}
    \pi_d(v_{target}) = \sum_{i=1}^{N} \frac{\theta_{id} \times w(v_i, v_{target})}{\sum_{i=1}^{N} w(v_i, v_{target})}
\end{equation}

Finally, the segregation index ($SI_D$) is computed using the equation below, normalized to range between 0 and 1 by the factor $\frac{n}{2n-2}$ (higher values indicate greater segregation):

\begin{equation}
\label{equation:segregation_index}
    SI_D(v_{target}) = \frac{n}{2n-2} \times \sum_{d \in D} \left| \pi_d(v_{target}) - \frac{1}{n} \right|
\end{equation}

\subsubsection{Bridging Index}
While traditional segregation indices highlight divisions, the bridging index (Fig.~\ref{fig:data_analysis}-A-2), proposed in~\cite{nilforoshan2023human} emphasizes opportunities for integration and connection.
It can identify possible ``bridges'' for social integration by computing the diversity of social groups interacting in a hub, assuming everyone visits their nearest hub.
However, due to limitations in our dataset, we adapt this concept by treating a CBG as a hub and focusing on the $k$ nearest CBGs to each $v_{target}$, where $k$ is adjustable. 
We first estimate the proportion of residents from each group $d$ within these CBGs who might visit $v_{target}$, where $p(v_i)$ is the population size of a source CBG $i$:

\begin{equation}
    \pi_d(v_{target})\prime = \sum_{i=1}^{k} \frac{\theta_{id} \times p(v_i)}{\sum_{i=1}^{k} p(v_i)}
\end{equation}

Then, we measure the bridging index ($BI_D$),  using the following equation, which is the inverse of the segregation index:

\begin{equation}
\label{equation:bridging_index}
    BI_D(v_{target}) = 1 - \frac{n}{2n-2} \times \sum_{d \in D} \left| \pi_d(v_{target})\prime - \frac{1}{n} \right|
\end{equation}

\begin{figure*} [t!]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/system_v1.png}
 \vspace{-0.5cm}
 \caption{
     The interface of \systemname guides experts through a segregation analysis and iterative intervention design workflow. 
     In the \commview (A), experts analyze the sociodemographic profiles and interconnections of mobility-based communities, identifying areas with potential segregation.
     Experts then drill down into the \cbgview (B) to select a target CBG for intervention, investigating how its features influence inflow patterns from different social groups.
     Meanwhile, the \mapview (C) offers geographic context for these mobility patterns.
     Finally, experts use the \whatifview (D) to simulate urban planning interventions, with the predicted impact of those changes reflected directly in the \cbgview (B) and the \mapview (C).
 }
 \vspace{-0.4cm}
 \label{fig:system-visual}
\end{figure*}

\subsubsection{Dual-Attribute Ranking}
\label{sec:TOPSIS_ranking}
Research by Nilforoshan \et~\cite{nilforoshan2023human} highlights a strong inverse relationship between bridging and segregation indices.
While relocating residents to bridge different social groups is beneficial, it is too ethically complex and thus impractical for our study~\cite{sanbonmatsu2011moving}. 
In consultation with our expert, we shifted focus towards CBGs with high bridging index (diverse neighborhoods) yet still experiencing high segregation.
These offer the potential for interventions to increase visitor diversity.

Therefore, a Multi-Criteria Decision Making (MCDM) method can help us more easily prioritize the CBGs with both high segregation index $SI$ and bridging index $BI$.
This approach is crucial for prioritizing CBGs for intervention and for organizing them in the \cbgTable discussed in Section~\ref{vis:cbg_view}. 
Among various MCDM techniques, we selected the Technique for Order of Preference by Similarity to the Ideal Solution (TOPSIS)~\cite{lai1994topsis} for its simplicity and effectiveness.
TOPSIS ranks CBGs based on their proximity to both ideal (high $BI$ and $SI$) and negative-ideal (low $BI$ and $SI$) benchmarks (Fig.~\ref{fig:data_analysis}-A-3). 
It effectively surfaces CBGs that not only are positioned well for fostering integration but also currently suffer from high segregation.

\subsection{Mobility Data Modeling}

\subsubsection{Deep Learning Model}
\label{sec:model}
We develop a deep learning model adapted from Deep Gravity~\cite{simini2021deep} (Fig.~\ref{fig:data_analysis}-B-1), the state-of-the-art deep learning framework designed to predict mobility flows based on environmental features including distance, population size, land use, and densities of different types of POI.
We made two key adaptations for segregation analysis, with the effectiveness evaluated in Section~\ref{sec:model_evaluation}:
\begin{itemize}
    \item Social group segmentation: 
        We divide the \textit{Mobility Dataset} ($G$) into segments ($G_d$) for each social group $d \in D$, enabling separate models to capture group-specific mobility patterns.
    \item Visitor characteristics inclusion:
        Inspired by Moro \et~\cite{moro2021mobility} that models the preference of people to visit the places where they are the minority in visitors, we include the sociodemographic characteristics of visitors computed using Equation \ref{equation:segregation_prop} as part of the input vectors. 
        This aims to model how different social groups respond to the visitor characteristics of a destination area.
\end{itemize}

Our adapted model's input for an origin-destination CBG pair $(v_i, v_j)$ is $concat[p_i, p_j, x_i, x_j, \pi_j, dis_{i,j}]$, where $p_i$, $p_j$ are the population sizes, $x_i$, $x_j$ represent densities of different types of POIs of the origin and destination, $\pi_j$ is a vector for the visitor characteristics of the destination, and $dis_{i,j}$ is their geographical distance. 
We employ a neural network architecture consistent with the original Deep Gravity model consisting of 15 hidden layers, combining wider layers (256 neurons) and narrower layers (128 neurons) with LeakyReLU activations.
The network predicts a mobility likelihood score $s(v_i, v_j)$ for each origin-destination CBG pair. For each origin CBG $v_i$, it calculates these scores for $k$ randomly selected destinations, and here $k$ is set to be 30 to speed up the computation.
The likelihood scores are transformed into predicted probabilities using the softmax function, and the predicted flow volume from $v_i$ to $v_j$, $\hat{w}(v_i, v_j)$, is calculated by multiplying the total number of individuals from $v_i$ to its $k$ destinations with its probability:

\begin{equation}
    \hat{w}(v_i, v_j) = \left( \sum_{l=1}^{k} w(v_i, v_l) \right) \cdot \frac{e^{s(v_i, v_j)}}{\sum_{l=1}^{k} e^{s(v_i, v_l)}}
\end{equation}

\subsubsection{Partial Dependence Plots}
\label{sec:model_pdp}
To understand how individual features influence predictions within our deep learning models, we utilize Partial Dependence Plots~\cite{hastie2009elements, friedman2001greedy} (Fig.~\ref{fig:data_analysis}-B-2).
PDP is a popular explainable AI technique for delineating the influence of individual features on the model's output, which is the predicted likelihood scores of mobility in our case.
While other XAI techniques like SHAP~\cite{lundberg2017unified} and LIME~\cite{ribeiro2016should} exist, they offer more granular insights into individual predictions.
In contrast, PDP aligns more with our goal of understanding the general trends of how various environmental and sociodemographic features impact the mobility patterns of different social groups.
We utilize \verb|sklearn.inspection.partial_dependence| to compute the partial dependence.
For the trained model of each social group, we generate line plots for the POI and visitor characteristics-related features of the destination CBG  $v_j$, \ie, $x_{j}$ and $\pi_{j}$, and obtain sets of x-values (feature values) and corresponding y-values (predicted impact).

\subsubsection{What-If Analysis}
\label{sec:model_what_if}
To allow users to explore the potential impact of hypothetical urban planning changes on mobility patterns, we develop a What-If Analysis module to enhance the deep learning model (Fig.~\ref{fig:data_analysis}-B-3).
When some POI-related features in the target CBG ($v_{target}$) are modified as $x_{target}\prime$, the function modifies the input vector for each pair of origin and target CBG $(v_i, v_{target})$, resulting in a new set of input vectors $concat[p_i, p_{target}, x_i, x_{target}\prime, \pi_{target}, dis_{i,{target}}]$.
These modified vectors are then fed to our trained models to predict new mobility flows \(\hat{w}_{after}(v_i, v_{target})\) from different social groups.
To quantify the impact of the change, we calculate the difference between the predicted flows before and after the hypothetical intervention using the equation below, and increment the predicted differences to actual flow volumes accordingly, as the new flow volumes resulting from feature adjustments:

\vspace{-0.5cm}
\begin{equation}
    \Delta \hat{w}(v_i, v_{target}) = \hat{w}_{after}(v_i, v_{target}) - \hat{w}_{before}(v_i, v_{target})
\end{equation}

==> archive/sections_for_vis24__old_/05_visual_design.tex <==
\section{Visual Design}
\label{sec:05_visual_design}

\systemname consists of four views to fulfill the analysis goals introduced in Section~\ref{sec:03_Background_VisualizationDesignTasks}: \commview (Fig.~\ref{fig:system-visual}-A), \cbgview (Fig.~\ref{fig:system-visual}-B), \mapview (Fig.~\ref{fig:system-visual}-C), and \whatifview (Fig.~\ref{fig:system-visual}-D).
We demonstrate the seamless analysis flow using the four views with an illustrative use case derived from our case studies:
A social scientist investigates income-based segregation in a city.
After analyzing the interconnection between detected mobility-based communities (\TIpill) and comparing their sociodemographic distributions (\TIIpill) in the \commview, he notices one with a significant low-income concentration, indicating segregation.
Drilling down into this community in the \cbgview, he identifies a target CBG with high segregation and potential for intervention (\TIIIpill).
Cross-referencing the target CBG's features in the \cbgview with inflow patterns in the \mapview, he observes a lack of health-related POIs in the target CBG, which could explain its limited appeal to higher-income groups (\TIVpill).
Finally, using the \whatifview to simulate an increase in such POIs, he receives feedback suggesting this intervention could reduce segregation (\TVpill).
% After identifying a segregated community of interest, \cbgview (Fig.~\ref{fig:system-visual}-B) helps pinpoint CBGs with potential for intervention (\TIIIpill).
% Meanwhile, \mapview (Fig.~\ref{fig:system-visual}-C) and \cbgview work together to reveal how environmental features influence the inflows of different social groups to the target CBG (\TIVpill).
% Finally, \whatifview empowers experts to simulate urban planning changes and assess their potential impact on segregation (\TVpill), receiving real-time feedback in both \cbgview and \mapview.

\subsection{Community View}
The \commview (Fig.~\ref{fig:system-visual}-A) provides an overview for exploring mobility-based community structures within the city and their sociodemographic characteristics.
It allows experts to customize the city and attribute of interest and the flow threshold, and detect communities using the Leiden algorithm as described in Section~\ref{sec:community_detection}.
Then, it supports the comparison of community sociodemographic profiles using the \commsig (Fig.~\ref{fig:system-visual}-A1) (\TIIpill) and inter-community flows in the \flowmat (Fig.~\ref{fig:system-visual}-A2) (\TIpill).
Finally, experts can indicate a community of interest for the following analysis.

\textbf{\commsig.}
To support the efficient analysis of the sociodemographic profiles of detected communities, a \commsig of each attribute accompanies each community, displayed in its corresponding color (\TIIpill).
The top row features the signatures of the chosen attribute, while subsequent rows provide additional attribute signatures as auxiliary information.
A signature (Fig.~\ref{fig:signature}-A) resembles horizontally aligned boxplots (Fig.~\ref{fig:signature}-B), with only the interquartile range (IQR) preserved and linked by smooth lines.
Within each IQR box in a signature, its height represents the range of proportions for a social group within the central 50\% of CBGs in the community, with the median line highlighted in a darker color for emphasis
A detailed legend about the signatures of an attribute will be shown upon hovering over the question mark icon beside the attribute name.

\textit{Justification:}
We initially displayed distributions using traditional boxplots (Fig.~\ref{fig:signature}-B). 
However, our domain expert found them visually overwhelming when comparing sociodemographic profiles across multiple communities. 
He suggested that at the early analysis stage, social scientists often focus on the distributions within the majority of CBGs in a community to gain an overall impression. 
Therefore, we designed the \commsig to emphasize the essential IQR information, representing the central concentration of CBGs, while simplifying the visual presentation.
Connecting IQRs with lines enhances visual continuity, aiding efficient comparison.
Our expert further recognized that this design streamlined his analysis, allowing him to rapidly identify similarities and differences between community attribute distributions based on the signature shapes.
% We originally adopted a traditional way to display the distributions by boxplots (Fig.~\ref{fig:signature}-B). 
% However, while boxplots offer detailed distribution data, they can become visually overwhelming when used in multiples. 
% After consulting to our domain expert, he mentioned that social scientists may only focus on the distributions of majority CBGs in an large area, 
% The \commsig design retains the essential IQR information and the median value for each social group while streamlining the visual presentation.
% Furthermore, IQRs are connected with lines which enhance visual continuity, facilitating the efficient analysis of community socioeconomic profiles.

\begin{figure} [t]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/design-signature.png}
 \vspace{-0.5cm}
 \caption{
     (A) The income \commsig design to show the income distributions of CBGs in community B. 
     (B) shows an alternative design: traditional boxplots.
     (C) The visual encoding of a cell in the \flowmat.
 }
 \vspace{-0.4cm}
 \label{fig:signature}
\end{figure}

\textbf{\flowmat.}
The \flowmat visualizes inter-community mobility patterns within the city (\TIpill), which has been segmented into N communities.
This $(N+1) \times (N+1)$ matrix resembles the adjacency matrix of a directed weighted graph. 
In the matrix, rows represent community outflows, columns represent inflows, and the final column/row depicts total flows.
Each matrix cell (Fig.~\ref{fig:signature}-C) encodes the visitor flow between two communities, and bars within the cell represent the proportions of different social groups (consistent with the encoding in the \commsig).
A log-normalized scale represents flow volume through the background color of the bars, and the flow volume can be aggregated as mean, median, sum, and standard deviation via the ``Flow aggregation'' selector above. 
Community labels on the left act as selectors for experts to choose a community of interest.

\textit{Justification:}
While a node-link visualization was considered, we adopted the matrix representation to visualize the multivariate flows and their attributes for its effectiveness of matrices for comparing edge attributes~\cite{nobre2019state, alper2013weighted}.
In our case, these attributes represent the crucial distribution of social groups within the flows between communities.

\subsection{CBG View}
\label{vis:cbg_view}
The \cbgview (Fig.~\ref{fig:system-visual}-B) comprises two components for detailed CBG-level analysis:
(1) the \cbgTable (Fig.~\ref{fig:system-visual}-B2) to identify CBGs with intervention potential for mitigating segregation within a chosen community (\TIIIpill);
(2) the \radar (Fig.~\ref{fig:system-visual}-B3) helps experts explore how environmental features influence the inflows from different social groups to a target CBG (\TIVpill).

\textbf{\cbgTable.}
An interactive \cbgTable inspired by the Ranking View in SmartAdp~\cite{liu2016smartadp} displays a list of CBGs ranked by TOPSIS, as described in Section~\ref{sec:TOPSIS_ranking}, that prioritizes the CBGs in diverse neighborhoods but experiencing high segregation (\TIIIpill).
Each row showcases a CBG with the geographical boundary shape, segregation index $SI$ and bridging index $BI$ (with bars representing their magnitudes), and proportions of social groups behind these two indices (encoded with bar charts consistent with the \flowmat).
Experts can adjust the $k$ neighbors parameter to modify the bridging index calculation and reorder the table (Fig.~\ref{fig:system-visual}-B1).
Selecting a CBG row will set it as the target CBG, allowing detailed feature impact exploration in the \radar and inflow pattern analysis in the \mapview.
% Furthermore, in the later introduced What-If View phase, the rows become expandable to reveal the impact of user-defined intervention strategies on the CBG.

\textbf{\radar.}
A radar chart, integrated with paired PDP area charts, reveals how the target CBG's features influence the inflows from different social groups (\TIVpill).
Each axis radiating from the center represents a feature of the target CBG, with two colored PDP area charts on either side showing the relationship between the feature value and the predicted impact of that feature on selected social groups (\eg, people in ``Under \$50K'' and ``Over \$200K'' income groups).
Each area chart (Fig.~\ref{fig:system-visual}-B4) is generated from the deep learning model's Partial Dependence Plots (PDP) (Section~\ref{sec:model_pdp}).
The x-axis encodes the feature value, and the y-axis indicates the predicted mobility likelihood. 
A larger area indicates a more significant impact in attracting visitors from that social group.
Meanwhile, a radar line overlaid on the area charts visualizes the target CBG's actual feature values.
For example, the larger area for the ``Over \$200K'' group on the shopping POI axis suggests wealthier people are more likely to visit CBGs with abundant shopping facilities.
The radar line's low value on this axis further indicates a lack of such amenities in the target CBG, offering a potential explanation for the limited inflow from higher-income individuals.

\textit{Justification:}
We chose the radial layout for the PDP charts over traditional vertical alignment for its following advantages.
First, the radial layout is a more common representation of place-based features in visualization literature~\cite{zeng2017visualizing, liu2016smartadp}, enhancing familiarity and making the design more compact.
Second, it provides variation from the vertically aligned bar charts elsewhere in the interface, promoting visual harmony. Our domain expert also confirmed that the radial layout improves the overall aesthetic appeal of the design.

\begin{figure} [t]
 \centering 
 \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figs/design-glyph.png}
 \vspace{-0.5cm}
 \caption{
     (A) The \bubbleglyph design to demonstrate one CBG's resident sociodemographics and flow patterns to target CBG.
     (B) and (C) show two alternative glyph designs.
 }
 \vspace{-0.4cm}
 \label{fig:glyph}
\end{figure}

\subsection{Map View}
\label{vis:map_view}
The \mapview (Fig.~\ref{fig:system-visual}-C) provides geographical information, juxtaposing the \realmap (Fig.~\ref{fig:system-visual}-C1) for geographical context for the detected communities (\TIpill) and the \dorlingmap (Fig.~\ref{fig:system-visual}-C2) to analyze the detailed flows between CBGs (\TIVpill).

\textbf{\realmap}. It displays the city's map with color-coding CBGs according to their community assignment. It offers two modes: ``full mode'' reveals the entire city, while ``focus mode'' highlights a selected target CBG (in black) and its closest $k$ neighbors, where $k$ adjusts based on settings in the \cbgTable of the \cbgview (Section~\ref{vis:cbg_view}).

\textbf{\dorlingmap}. It employs a Dorling layout~\cite{dorling1996area} to preserve relative CBG positions to allow more informative representations of the target CBG and its neighbors by glyph encoding.
Specifically, a \bubbleglyph (Fig.~\ref{fig:system-visual}-C3) visualizes the detailed information of a CBG.

\textbf{\bubbleglyph.}
Inspired by the concept of social filter bubbles that isolate people into homogeneous individuals, we designed the metaphor-based \bubbleglyph to showcase one CBG's resident demographics and flow patterns, as shown in Fig.~\ref{fig:glyph}.
The background color of the glyph matches the CBG's assigned community, and the glyph's radius represents the population size of the CBG.
The CBG's actual geographical boundary shape is at the center inside the glyph to aid in connecting with \realmap and \cbgTable.
A circle of white proportion arcs around the shape represents the proportions of different social groups in the CBG's resident population.
The arcs resemble the reflection light on a bubble: the dominance of one arc will create a bubble-like appearance, visually indicating segregation.
When an arc is hovered, its full axis will show the maximum possible length of the arc, with a tooltip showing the detailed group name and proportion values.
A thicker flow arc around the boundary represents the proportion of residents visiting the target CBG.
% Its length is determined by the following equation: \begin{equation} p = \frac{w(v_i, v_{target})}{\sum_{l=1}^{N} w(v_i, v_l)} \end{equation}
% During the What-If phase, a thinner gold arc within the original arc visualizes the predicted flow proportion changes resulting from interventions.

\textit{Justification:}
We designed the bubble glyph after carefully considering several alternatives (Fig.~\ref{fig:glyph}-B, C).
Design B uses circular distributions around the circle boundary to represent the proportions of social groups. However, our expert found it not very effective to compare across different CBGs by the area of the distributions.
Additionally, their height can become large in cases of extremely segregated CBGs, wasting space and potentially causing confusion with the radius that represents population size.
Design C places flow information as a bar chart consistent with \flowmat, which saves space.
However, this layout limits the flow arc to less than a full circle, which is counter-intuitive and potentially misleading for chart reading.
Furthermore, our domain expert also favored the \bubbleglyph the most as it is intuitive and aesthetically pleasing, and the metaphor-based design can vividly remind him of segregation. 

\subsection{What-If View}
The \whatifview (Fig.~\ref{fig:system-visual}-D) enables users to design hypothetical interventions for reducing segregation in the target CBG (\TVpill).
It provides sliders for users to adjust features (\ie, the density of specific POIs). 
Changes are then dynamically fed into the deep learning model's What-If Analysis module (Section~\ref{sec:model_what_if}) to predict the new mobility patterns of different social groups after interventions, triggering updates across visualization components.

\textbf{Predictions and Feedback.}
This view serves as the central hub for experimentation, interacting with other visualization components to provide real-time feedback on the interventions with details below, facilitating strategy evaluation and refinement.

\cbgTable (Section~\ref{vis:cbg_view}): When a CBG's features are modified, its corresponding row will become expandable, with sub-rows representing intervention strategies (Fig.~\ref{fig:system-visual}-B2).
Predicted changes to the segregation index and inflow proportions of social groups are visualized with thin gold bars overlaying the original bars. 
Users can save, edit, and delete strategies using the icons on the right side. 

\radar (Section~\ref{vis:cbg_view}): A dashed radar line will appear alongside the original one, showing the target CBG's features after the intervention (Fig.~\ref{fig:system-visual}-B3). 

\dorlingmap (Section~\ref{vis:map_view}): In glyphs, thinner gold flow arcs (consistent with the color in the \cbgTable) will overlay the original flow arcs to visualize flow changes resulting from interventions (Fig.~\ref{fig:system-visual}-C3).

% In \cbgTable, with each strategy sub-row showing the detailed change in the segregation index and inflow proportions of each user-defined intervention strategy, with thin gold bars on the top of the original bars to represent the new predicted index and proportions (\TVpill). Experts can also view, edit, and delete strategies by clicking the icons at the right side of each strategy sub-row.

==> archive/sections_for_vis24__old_/06_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we present a quantitative analysis of the effectiveness and complexity of our deep learning model. 
Then, we demonstrate two case studies developed with our experts.
We invited $E_B$, a marketing data scientist with three years of experience in income-based segmentation, to explore case 1 about income segregation.
We then invited our domain expert $E_A$, introduced in Section~\ref{prob_formulation}, to explore case 2 about partisan segregation.
Besides, we invited two more experts ($E_C$ and $E_D$) for the expert interviews detailed in Section~\ref{design_implication}.
$E_C$ has four years of experience in Geographical Information Systems (GIS), focusing on agent-based modeling (ABM) of segregation.
$E_D$ is a doctoral student who has been researching segregation on social media for two years.

\subsection{Model Evaluation}
\label{sec:model_evaluation}

\parasum{Effectiveness of adaptation.}
% \subsubsection{Effectiveness of adaptation}
To assess our adaptations to the original Deep Gravity model (social group segmentation and visitor characteristics inclusion as described in Section \ref{sec:model}), we ran a comparison experiment with four settings: 
the original Deep Gravity (DG) model as a baseline, DG + Social Groups (adding social group segmentation), DG + Visitor (including visitor characteristics), and our adopted version, DG + Social Groups + Visitor (combining both adaptations).
Consistent with case 1, we used Houston data, segmented social groups by income, and included income and race as visitor characteristics
All models were trained for 10 epochs (repeated 20 times).
We then employed the Common Part of Commuters (CPC) metric using the following equation, consistent with the original work~\cite{simini2021deep}, to compare predicted flow $\hat{w}(v_i, v_j)$ with ground truth flow $w(v_i, v_j)$.

\begin{equation}
    CPC(v_i, v_j) = \frac{2 \sum_{i,j} min(\hat{w}(v_i, v_j), w(v_i, v_j))}{\sum_{i,j} \hat{w}(v_i, v_j) + \sum_{i,j} w(v_i, v_j))}
\end{equation}

Results (Table \ref{tab:algo-results}) confirm the validity of both adaptations. Our adopted setting achieved the highest CPC score.

\begin{table}[h!]

\centering
\vspace{-0.2cm}
\begin{tabular}{l|cc}
\toprule
\textbf{Model setting} & \textbf{Mean CPC} & \textbf{Std. Dev. CPC} \\
\midrule
DG (Baseline)                     & 0.6007 & 0.0850 \\ 
DG + Social Groups                & 0.6049 & 0.0837 \\ 
DG + Visitor      & 0.6069 & 0.0852 \\ 
DG + Social Groups + Visitor            & \textbf{0.6117} & \textbf{0.0854} \\ 
\bottomrule
\end{tabular}
\vspace{-0.2 cm}
\caption{Performance comparison across different model settings}
\vspace{-0.7 cm}
\label{tab:algo-results}
\end{table}


\parasum{Time complexity.}
% \subsubsection{Time complexity}
We performed model training and inference on a 16GB MacBook Pro (Apple M1, no GPU). 
For Houston (around 2000 CBGs), in our case, individual model training took approximately 1 minute. 
Therefore, we pre-trained models with expert-identified features and computed PDPs offline. 
Model inference during what-if analysis (Section \ref{sec:model_what_if}) was fast (typically within 2 seconds), ensuring real-time interface feedback.

\begin{figure*} [t!]
 \centering 
 \vspace{-0.5cm}
 \includegraphics[width=\linewidth]{figs/case_v0.png}
 \vspace{-0.5cm}
 \caption{
     Case 2 - \systemname guided expert $E_A$ in analyzing partisan segregation and designing interventions. 
     He first compared the sociodemographics of communities (A1, A2) and searched for promising CBGs with intervention potential (B1, B2).
     He then analyzed the partisan preferences in mobility to the target CBG (B3, C1).
     He tried increasing food-related POIs (D1) to attract diverse visitors but it surprisingly worsened segregation (B4, C2).
     In contrast, increasing shopping facilities (D2) reduced segregation (B5).
     Finally, a combined intervention (D3) proved most effective (B6, C3).
 }
 \vspace{-0.6cm}
 \label{fig:system-case}
\end{figure*}

\definecolor{commAColor}{HTML}{51c44a} %6acc64
\definecolor{commBColor}{HTML}{4878d0}
\definecolor{commEColor}{HTML}{8c613c}
\newcommand{\commA}{Community \textcolor{commAColor}{\textbf{A}}\xspace}
\newcommand{\commB}{Community \textcolor{commBColor}{\textbf{B}}\xspace}
\newcommand{\commE}{Community \textcolor{commEColor}{\textbf{E}}\xspace}
% \newcommand{\commA}{Community \tcbox[on line, colframe=commAColor, colback=commAColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{A}\xspace}
% \newcommand{\commB}{Community \tcbox[on line, colframe=commBColor, colback=commBColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{B}\xspace}
% \newcommand{\commE}{Community \tcbox[on line, colframe=commEColor, colback=commEColor,coltext=white,
% arc=0mm, boxsep=0mm, left=1pt, right=1pt, top=1pt, bottom=1pt, boxrule=0.3mm]{E}\xspace}

\subsection{Case Studies}
Our cases focus on understanding and mitigating urban segregation in Houston City, the fourth-most populous city in the United States, known for its income inequalities~\cite{houstonincome} and partisan polarization~\cite{houstonpartisan}.

\subsubsection{Case1: A Prescription for Income Harmony}
We invited $E_B$, an experienced marketing data scientist working on income-based segmentation, to explore the first case about \textbf{income segregation}.
The income attribute uses the census data from 5-year American Community Survey and classifies the income into four groups from low to high: ``Under \$50K'', ``\$50K - \$100K'', ``\$100K - \$200K'', and ``Over \$200K''.
As suggested by $E_B$, the visitor characteristics in the input feature include both race and income.

\textbf{Overview of income disparities.} 
$E_B$ compared income signatures (\TIIpill) in the \commview (Fig. \ref{fig:system-visual}-A), and \commB (blue) emerged with a distinct segregation profile, characterized by a significant first box representing the low-income population (Fig. \ref{fig:system-visual}-A1-2).
In contrast, \commA (green), adjacent to Community B, exhibits greater economic diversity, with its signature showing a more even distribution across groups (Fig. \ref{fig:system-visual}-A1-1).
The \realmap (Fig. \ref{fig:system-visual}-C1) helped him localize them: \textit{``Community B is north of downtown, where neighborhoods face high poverty; Community A is located southwest of downtown, with booming areas like Sugar Land.''}

He then turned to the \flowmat (Fig. \ref{fig:system-visual}-A2) to understand inter-community connections (\TIpill), finding that Community B displays the most extreme income segregation in both incoming (last row) and outgoing (last column) mobility patterns.
Additionally, the lighter background shading of Community A's flow bar chart indicates minimal interaction with Community B.
\textit{``Despite their proximity, these communities rarely interact, deepening the segregation in activity spaces. How can we bridge this divide?''} $E_B$ wondered.
Therefore, he clicked Community B's label in the left column to focus on Community B.

\textbf{Targeting a CBG for intervention.}
Targeting specific CBGs within Community B for interventions (\TIIIpill), $E_B$ utilized the \cbgTable (Fig. \ref{fig:system-visual}-B2), focusing on those with high segregation and bridging indexes.
Selecting the first CBG as the target triggered a series of visual updates: it was highlighted in black on both the \cbgTable and \realmap.
The \radar (Fig. \ref{fig:system-visual}-B3) and \dorlingmap (Fig. \ref{fig:system-visual}-C2) also updated, displaying the chosen CBG's features and neighborhood connections.
On the \realmap, noticing its position at the boundary between Community A and Community B, $E_B$ tried increasing the top $k$ neighbors parameter from 20 to 30 (Fig. \ref{fig:system-visual}-B1) to broaden his analysis scope.

\textbf{Analyzing inflow patterns and revealing intervention needs.}
$E_B$ further delved into inflow patterns to the target CBG, aiming to uncover the reasons behind its segregation (\TIVpill).
The \dorlingmap's \bubbleglyph (Fig. \ref{fig:system-visual}-C2) revealed a common trend: the target CBG and neighboring CBGs within Community B all showed a dominance of the lowest income group (indicated by the longest white arc).
In contrast, five CBGs on the target CBG's west side from Community A exhibited a more balanced distribution across income groups.
Meanwhile, the inter-community differences existed in inflow patterns. 
Comparing the flow arcs, $E_B$ observed a significantly higher volume of visitors from CBGs within Community B compared to those from Community A.

To pinpoint the features influencing these mobility patterns, he compared the ``Under \$50K'' and ``Over \$200K'' groups within the \radar (Fig. \ref{fig:system-visual}-B3).
The Partial Dependence Plot (PDP) bars revealed distinct preferences among income groups.
After comparing the PDP wings and radar line for $R_w$, $R_b$, and $R_h$, $E_B$ reasoned: \textit{``Wealthier visitors prefer homogeneous, predominantly White areas, avoiding areas with high Black and Hispanic visitor proportions, such as this target CBG.''} 
Regarding POI impact, he identified a lack of health-related amenities as a potential reason for the limited appeal to a wealthier demographic. \textit{``There is also a gap in meeting the needs of a high-value market segment, reinforcing segregation.''}

\textbf{Testing an intervention strategy for integration.}
Inspired by his findings, $E_B$ turned to the \whatifview (Fig. \ref{fig:system-visual}-D) to design an intervention aimed at reducing income segregation (\TVpill).
Using the slider, he simulated an increase in health-related POIs within the target CBG, raising the density from zero to 3.5 units per square kilometer. 
The simulated outcome was promising - the \cbgTable's expanded row indicated a predicted 3.15\% decrease in segregation. Additionally, the \dorlingmap visualized an increased flow from Community A to the target CBG, depicted by longer gold arcs.
\textit{``This highlights the importance of strategic placement,''} $E_B$ concluded, \textit{``Adding resources isn't enough – it's about targeting them to bridge communities. Much like expanding a product line to attract a wider customer base.''}

This case demonstrates how \systemname assists in understanding the urban segregation landscape, its possible causes, and how to design data-driven interventions. 
While tailored for social science, this example highlights the system's value for other fields, like marketing, where attracting diverse groups is a strategic goal.

\subsubsection{Case2: From Partisan Lines to Shared Spaces}
We invited $E_A$, our domain expert focusing on political polarization research, to explore the second case about \textbf{partisan segregation}.
For this analysis, we used the L2 Political Academic Voter File to obtain partisan membership data.
We classified non-Democratic or Republican parties as either ``Lean Democrat'' or ``Lean Republican,'' excluding independent or non-partisan individuals.
Proportions of these two partisan groups were then calculated for each CBG and included in the Sociodemographic Dataset (as described in Section \ref{sec:data_abstraction}). 
Following $E_A$'s suggestion, both income and partisan memberships were used as visitor characteristics in the input data to reveal the interplay between income levels and political beliefs.

\textbf{Searching for CBGs with intervention opportunities.}
After segmenting the city into communities (\TIpill), $E_A$ navigated through each community searching for CBGs with intervention opportunities (\TIIpill{}, \TIIIpill). 
\commB (blue), predominantly Lean Democrat, initially caught his eye (Fig. \ref{fig:system-case}-A1). 
However, a closer look revealed a lack of CBGs with both a high segregation index and a high bridging index (Fig. \ref{fig:system-case}-B1), making it less ideal for his intervention plan.
Redirecting his focus, $E_A$ discovered \commE (brown), a politically mixed area (Fig. \ref{fig:system-case}-A2) with a promising landscape, with several CBGs flagged for both high segregation and bridging potential (Fig. \ref{fig:system-case}-B2). 
Therefore, he selected Community E and chose its first CBG for in-depth analysis.

\textbf{Analyzing partisan preferences in mobility.}
In assessing the reasons that cause inflow patterns via the \radar (Fig. \ref{fig:system-case}-B3) and the \dorlingmap (Fig. \ref{fig:system-case}-C1) (\TIVpill), $E_A$ observed a pronounced Democratic lean within the target CBG. 
Notably, adjacent Republican-leaning CBGs on the west side exhibited negligible inflow, underscoring existing political divides.

In his analysis of the PDP wings, $E_A$ observed distinct behaviors in relation to the feature $P_D$ (the proportion of ``Lean Democrat'' visitors in a CBG), highlighting a trend where ``Lean Democrat'' individuals prefer visiting areas with a Democrat majority, whereas ``Lean Republican'' individuals tend to avoid these same places. 
Regarding the feature $P_R$ (the proportion of ``Lean Republican'' visitors in a CBG), the PDP wings indicated similar preferences between the two groups towards Republican-majority areas. 
$E_A$ reasoned, \textit{``This could be because areas with a Republican majority are less prevalent, making them less distinctive as political territories, or because Democrats, being the majority, might not perceive visiting Republican-majority areas as a threat to their social identity.''}
Furthermore, while both groups displayed similar preferences for POIs overall (Fig. \ref{fig:system-case}-B3), $E_A$'s domain expertise led him to suspect more nuanced dynamics: \textit{``Although they have a similar preference on the POIs, they may prefer different POIs depending on whether the area is dominated by their own party or the opposing party. This is what we call the `interaction effect'.''}

\textbf{Exploring synergies to bridge divides.}
Eager to examine the interaction between various features and find a suitable intervention strategy that leverages such interaction to reduce the partisan segregation in the target CBG, $E_A$ turned to the \whatifview (\TVpill).
He began by increasing the food facility density to 3 units per square kilometer (Fig. \ref{fig:system-case}-D1). 
Surprisingly, this action resulted in a 6.44\% increase in the segregation index (\ref{fig:system-case}-B4).
Examining the \dorlingmap (Fig. \ref{fig:system-case}-C2), he observed,
\textit{``While we saw an increase in visitors from Republican-dominant CBGs, there was also a surge in visitors from the Democrat-dominant CBGs around our target, which worsened the segregation. 
That reminds me of some policies intended to enhance minority engagement that unintentionally end up attracting a larger majority presence.''}

Resetting the current intervention, $E_A$ increased shopping facility density, noting a slight reduction in segregation. Advancing to 4 units per square kilometer (Fig. \ref{fig:system-case}-D2), he witnessed a 2.96\% drop in segregation (Fig. \ref{fig:system-case}-B5), with a notable increase in Republican-leaning visitors.
\textit{``This demonstrates the interaction I mentioned earlier. Though both food and shopping facilities can attract visitors, they have unique characteristics. Shopping facilities can attract more diverse people even if they are in a segregated place, but food facilities seem to only attract more segregated visitors in this case. Some existing literature also shows different POIs have different contributions to segregation~\cite{zhang2023human}. Places that require more face-to-face interaction, in this case, restaurants, may be more segregated.''} $E_A$ commented.
$E_A$ recorded this intervention and continued his exploration.

Intrigued by the interaction between shopping and food POIs, he simultaneously increased both types of amenities: shopping to 4 units per square kilometer and food to 3 units per square kilometer (Fig. \ref{fig:system-case}-D3).
Interestingly, this time, the segregation index did not increase because of the food facilities, but conversely, it decreased by 3.84\% (Fig. \ref{fig:system-case}-B6).
From the updated \dorlingmap (Fig. \ref{fig:system-case}-C3), it could be seen that Republican-dominated CBGs on the west side had more significant increases in visitor proportions to the target CBG.
\textit{``I thought the change would be linear and counteracted, but I didn't expect their combined effect to further decrease the segregation,''} $E_A$ pondered.
\textit{``In the previous research, we always treat POIs individually, and the combined effect of POIs is rarely touched, but such effect seems to be captured by the deep learning model here. I suspect that's because those facilities co-create shared experiences of consumption and leisure, making the target CBG an even more inclusive multi-use community center for people holding different political beliefs.''}
Finally, $E_A$ thanked the system for shedding light on his future research: \textit{``This is a truly interesting finding, and in my following study, I may focus on the effect of mixed-use area in the partisan segregation.''}

In summary, this case highlights that \systemname can help experts develop data-informed and feedback-driven urban planning insights to promote political integration and help researchers gain new insights that can be hard to reveal with traditional social science workflow.

==> archive/sections_for_vis24__old_/07_discussion.tex <==
\section{Discussion}
The two case studies demonstrate the usability and effectiveness of \systemname in helping experts understand and mitigate different types of urban segregation.
To enrich our findings further, we interviewed two more experts ($E_C$ and $E_D$).
We presented the case study results and invited them to explore the system freely, collecting their feedback.
% $E_C$ specializes in Geographical Information Systems (GIS) with a focus on agent-based modeling (ABM) of human mobility.
% Meanwhile, $E_D$ is a doctoral student in social science, focusing on online segregation.

\subsection{Design Implications}
\label{design_implication}
Below, we discuss insights from the feedback of four experts.

\textbf{Applications and target users of \systemname.} 
All experts praised the usefulness of \systemname, suggesting its potential applications beyond its current user base.
For the \commpill unity and \cbgpill-level analysis, $E_B$ and $E_C$ highlighted the progressive workflow as an efficient tool that enables geospatial analysts to rapidly explore the complex mobility data within unfamiliar cities without extensive custom coding.
$E_D$ expected to utilize the \commview and \dorlingmap to visualize communities and echo chambers on online social media.

For the \poipill-level Analysis, $E_A$ and $E_B$ saw it as a bridge between researchers and decision-makers, offering benefits in various scenarios. 
$E_A$ shared a compelling example of using its simulation power to inform urban decision-making: 
% \textit{``If I could use this system to simulate the impact of a community center demolition and present it to the municipal office, the decision-making process might have been entirely different.''}
\textit{``Imagine using this system before the decision of demolishing a community center and sharing these simulations with the municipal office; it might influence discussions and planning decisions.''}
Besides social scientists, $E_A$ noted that social activists and NGOs who want to promote social well-being in their own communities could use the system to assess the potential impact of municipal policies.
$E_B$ underscored the system's value for professionals in fields like marketing.
He shared that he previously used TensorFlow's What-If tool for simulations but found its output limited and difficult to contextualize for clients. However, \systemname offers visually appealing results and intuitive comparisons,  greatly enhancing presentations.


\textbf{Transparency of the simulation.}
$E_C$, specializing in spatial agent-based modeling (ABM), praised the deep-learning model's ability to capture complex human behavior (in case 2).  However, he highlighted a key difference between deep learning and ABM: the issue of explainability. \textit{``ABM, while potentially oversimplifying human behavior, grants experts direct access to agent attributes and states~\cite{liu2022abm}, allowing for greater transparency and control over experiments.''}  
Therefore, for future projects targeting experts who value rigorous experimental control,  we suggest carefully balancing the benefits of deep learning models with the explainability of ABM.
One potential hybrid approach is integrating ABM into mobility data modeling, leveraging the complex behavior captured by deep learning~\cite{turgut2023framework}.

\textbf{Feasibility consideration in ``technology for social good.''}
Both $E_B$ and $E_C$ appreciated our careful consideration of the feasibility of urban planning interventions during the design phase. 
The focus on identifying areas with high potential (using TOPSIS ranking) and implementing targeted interventions was seen as a key strength for promoting a greater chance of real-world impact. 
This approach, prioritizing practical implementation, can be borrowed for other technology-for-social-good projects, helping to narrow down targets and increase feasibility.

\subsection{Limitations and Future Works}
We introduce the limitations of our system and future work plans.

\textbf{Lack of temporal dimension.}
Currently, \systemname operates on a static snapshot of urban mobility and segregation patterns, not accounting for temporal variations. 
Urban dynamics, such as commuter flows and seasonal changes, can significantly impact segregation patterns. 
In the future, we will extend our deep learning model to analyze time-series mobility data and incorporate visualization techniques such as the Spatio-Temporal Graphs~\cite{von2015mobilitygraphs} to capture the temporal dynamics of segregation patterns.

\textbf{Possible bias in the demographic composition of visitors.}
We currently infer visitors' sociodemographic characteristics based on residents' census data. While this is a common practice in social science~\cite{zhang2023human, athey2021estimating}, it can introduce bias.
% For example, wealthy people living in an economically diverse CBG might primarily visit wealthy areas. However, under our current method, we'd estimate they also visit places frequented by other residents of the CBG, potentially underestimating income segregation.
In the future, we aim to improve data accuracy by obtaining individual-level mobility data (\eg, telecommunication data~\cite{wu2015telcovis}) and integrating more fine-grained imputation methods, such as using housing prices~\cite{nilforoshan2023human} to infer sociodemographics.

\textbf{Coarse-grained POI categories.}
The current 12 broad POI categories limit the granularity of insights provided for policymaking.
$E_A$ and $E_B$ suggested the value of modeling fine-grained categories within the current main categories. For example, distinguishing between fast food and fine dining restaurants might reveal significant differences in their impact on mobility~\cite{garcia2024effect}. 
However, this presents a challenge due to the large number of fine-grained POI categories (approximately 200 in our current SafeGraph dataset).
In the future, we plan to work closely with social scientists to develop a refined POI taxonomy. This taxonomy will balance comprehensiveness with a focus on the subcategories most impactful to segregation, enabling more accurate modeling.

\textbf{Visual scalability.}
The \radar currently displays all POI and visitor characteristics-related features.  As the number of features increases (\eg, with finer POI categories), the visualization may become overwhelming.
To address this, we will introduce a feature importance ranking mechanism (such as SHAP~\cite{lundberg2017unified}) to prioritize the display of top features. Additionally, we will implement filtering and search tools for flexible exploration of feature impact.

\textbf{More contextual geographical information.}
$E_C$ highlighted the need for additional geographic layers to inform the feasibility of urban planning interventions.
This includes elements like transportation networks and natural resources.
In the future, we will develop a more advanced \mapview showing multi-layered GIS data to provide a richer context for more accurate decision-making during \poipill-level analysis.

==> archive/sections_for_vis24__old_/08_conclusion.tex <==
\section{Conclusion}
In this work, we introduce \systemname, a visual analytics system that leverages human mobility data to empower in-depth exploration and mitigation of urban segregation.
Our system combines a data analysis pipeline with an interactive interface featuring novel visualizations to support a three-level analysis workflow, enabling experts to examine segregation patterns from overview to detail and iteratively design feedback-driven urban planning interventions.
A quantitative evaluation demonstrates our model's accuracy in modeling mobility data and its capabilities for real-time interactive analysis.
Case studies and expert interviews further highlight \systemname's value in helping social scientists and policymakers uncover complex segregation patterns and design inclusive, equitable urban spaces.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

